On recurrence and ergodicity for geodesic flows on noncompact periodic polygonal surfaces

We study the recurrence and ergodicity for the billiard on noncompact polygonal surfaces with a free, cocompact action of $\Z$ or $\Z^2$. In the $\Z$-periodic case, we establish criteria for recurrence. In the more difficult $\Z^2$-periodic case, we establish some general results. For a particular family of $\Z^2$-periodic polygonal surfaces, known in the physics literature as the wind-tree model, assuming certain restrictions of geometric nature, we obtain the ergodic decomposition of directional billiard dynamics for a dense, countable set of directions. This is a consequence of our results on the ergodicity of $\ZZ$-valued cocycles over irrational rotations.

==> bill-fig1.tex <==
%%BoundingBox: 85 20 500 490

0.9 0.9 scale

/Times-Roman findfont 15 scalefont setfont
/x 50 def /y 100 def /tx 60 def /ty 90 def
/dep 150 def /zx 0 def /zy 0 def 

/u 205 def /v 270 def /tu 150 def /tv 150 def
/dep 150 def /zu 0 def /zv 0 def

0.2 setlinewidth 
/rect1 {
newpath
u v moveto u v tv add lineto stroke
u v tv add moveto u tu add v tv add lineto stroke
u tu add v tv add moveto u tu add v lineto stroke
u tu add v moveto u v lineto stroke} def

rect1

1.2 setlinewidth 
/rect {
newpath
x y moveto x y ty add lineto stroke
x y ty add moveto x tx add y ty add lineto stroke
x tx add y ty add moveto x tx add y lineto stroke
x tx add y moveto x y lineto stroke} def

/flur { /fsz 16 def 
/fsz1 10 def /fsz2 6 def
zx zy moveto 
zx fsz add zy fsz add lineto stroke
zx fsz add zy fsz add moveto
zx fsz2 add zy fsz1 add lineto stroke
zx fsz add zy fsz add moveto
zx fsz1 add zy fsz2 add lineto stroke } def

/flul { /fsz 16 def 
/fsz1 10 def /fsz2 6 def
zx zy moveto 
zx fsz sub zy fsz add lineto stroke
zx fsz sub zy fsz add moveto
zx fsz2 sub zy fsz1 add lineto stroke
zx fsz sub zy fsz add moveto
zx fsz1 sub zy fsz2 add lineto stroke } def

/fldl { /fsz 16 def 
/fsz1 10 def /fsz2 6 def
zx zy moveto 
zx fsz sub zy fsz sub lineto stroke
zx fsz sub zy fsz sub moveto
zx fsz2 sub zy fsz1 sub lineto stroke
zx fsz sub zy fsz sub moveto
zx fsz1 sub zy fsz2 sub lineto stroke } def

/fldr { /fsz 16 def 
/fsz1 10 def /fsz2 6 def
zx zy moveto 
zx fsz add zy fsz sub lineto stroke
zx fsz add zy fsz sub moveto
zx fsz2 add zy fsz1 sub lineto stroke
zx fsz add zy fsz sub moveto
zx fsz1 add zy fsz2 sub lineto stroke } def

/x0 250 def /y0 300 def 

/x x0 def /y y0 def rect
x 12 sub  y ty add  moveto (A) show
x tx add y ty add  moveto (B) show
x 14 sub  y 5 sub moveto (D) show
x tx 8 add add  y 8 sub moveto (C) show
x tx 5 add add y tx add  moveto (D) show
x tx 13 add add y tx -4 add add  moveto (1) show
x 6 add y tx add moveto (C) show
x 14 add y tx -4 add add moveto (1) show
/x x0 dep add def /y y0 dep add def rect
/x x0 dep sub def /y y0 dep sub def rect
/x x0 dep sub def /y y0 dep add def rect
/x x0 dep add def /y y0 dep sub def rect

0.4 setlinewidth
x0 tx add y0 moveto 
x0 dep tx add add y0 dep add lineto
stroke

0.4 setlinewidth
x0 tx add y0 tx add moveto 
x0 dep add y0 dep add lineto
stroke

0.4 setlinewidth
x0 y0 tx add moveto 
x0 tx dep sub add y0 dep add lineto
stroke

0.4 setlinewidth
/zx x0 30 add def /zy y0 ty add def flur flul

/zx x0 tx add def /zy y0 30 add def flur fldr

/zx x0 30 add def /zy y0 def fldr fldl

/zx x0 def /zy y0 30 add def fldl flul

0.4 setlinewidth
/x x0 dep add def /y y0 def rect
/x x0 dep sub def /y y0 def rect
/x x0 def /y y0 dep add def rect
/x x0 def /y y0 dep sub def rect

x0 tx add y0 40 add moveto 
x0 dep tx 40 sub add add y0 dep add lineto
stroke 
/zx x0 tx add def /zy y0 40 add def flur
/zx x0 dep tx 40 sub add add def /zy y0 dep add def fldr

copypage


==> bill-fig2.tex <==
%%BoundingBox: 85 20 500 490
0.75 0.8 scale newpath 20 200 moveto 600 200 lineto 1 setlinewidth
stroke /Times-Roman findfont 20 scalefont setfont 15 180 moveto (0)
show 595 180 moveto (1) show 310 180 moveto (1/2) show

/xx1 150 def /trFct { 20 350 moveto 20 200 lineto stroke

20 350 moveto xx1 350 lineto stroke

xx1 350 moveto xx1 200 lineto stroke

/Symbol findfont 20 scalefont setfont 160 180 moveto (b) show

310 50 moveto 310 200 lineto stroke 310 50 moveto xx1 290 add 50
lineto stroke xx1 290 add  50 moveto xx1 290 add 200 lineto stroke
xx1 292 add 180 moveto (b+1/2) }

def trFct show copypage


==> bill-fig3.tex <==
%%BoundingBox: 5 5 705 205

0.75 0.8 scale

newpath 0 200 moveto 990 200 lineto 1 setlinewidth stroke

/Times-Roman findfont 20 scalefont setfont

-15 180 moveto (0) show

/xx0 0 def /xx1 0 def /xx2 0 def /eps 0 def

/largB 80 def /zxx0 0 def /zxx1 largB def /zxx2 100 def

/baseH 200 def /deplH 150 def /haut 0 def /nHaut 0 def

/haut baseH deplH add def /nHaut baseH deplH sub def

% trace fonction

/trFct {

/xx0 zxx0 eps add def /xx1 zxx1 eps add def /xx2 zxx2 eps add def

xx0 baseH moveto xx0 haut lineto stroke

xx0 haut moveto xx1 haut lineto 2 setlinewidth stroke

xx1 haut moveto xx1 baseH lineto 1 setlinewidth stroke

xx2 baseH moveto xx2 nHaut lineto stroke

xx2 nHaut moveto xx2 largB add nHaut 2 setlinewidth lineto stroke

xx2 largB add nHaut moveto xx2 largB add baseH

1 setlinewidth lineto stroke

zxx0 200 add  baseH 10 add moveto zxx0 200 add baseH lineto stroke

} def

% Fin trace fonction

% trace fonction2

/trFct2 {

/xx0 zxx0 eps add def /xx1 zxx1 eps add def /xx2 zxx2 eps add def

xx0 baseH moveto xx0 haut lineto stroke

xx0 haut moveto xx1 haut lineto 2 setlinewidth stroke

xx1 haut moveto xx1 baseH lineto 1 setlinewidth stroke

xx2 baseH moveto xx2 nHaut lineto stroke

xx2 nHaut moveto xx2 largB add nHaut lineto 2 setlinewidth stroke

xx2 largB add nHaut moveto xx2 largB add baseH

1 setlinewidth lineto stroke

} def

% Fin trace fonction2

% write symb

/char1 (a) def /char2 (a) def

/wrSymb {/Times-Roman findfont 20 scalefont setfont

xx0 2 sub baseH 20 sub moveto (n) show

xx0 6 add baseH 30 sub moveto char1 show

/Symbol findfont 20 scalefont setfont

xx0 12 add  baseH 20 sub moveto char2 show

/Times-Roman findfont 20 scalefont setfont } def

% Fin write symb

/eps 0 def trFct

/Symbol findfont 20 scalefont setfont

zxx1 12 sub baseH 20 sub moveto (e) show

zxx1 4 sub baseH 32 sub moveto (1/2)show

zxx2 6 add baseH 20 sub moveto (e) show

zxx2 10 add  baseH 32 sub moveto (b)show

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/Times-Roman findfont 20 scalefont setfont

/eps -6 def trFct

/char1 (1) def /char2 (a) def wrSymb

zxx0 10 sub  baseH 20 add moveto (1/q) show

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/eps 10 def trFct

/char1 (2) def /char2 (a) def wrSymb

zxx0 10 sub baseH 20 add moveto (2/q) show

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/eps -6 def trFct

/char1 (3) def /char2 (a) def wrSymb

zxx0 10 sub baseH 20 add moveto (3/q) show

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

zxx0 10 sub baseH 20 add moveto (4/q) show

/eps 5 def trFct2

/char1 (4) def /char2 (a) def wrSymb

copypage


==> bill-fig6.tex <==
%%BoundingBox: 5 5 705 490

0.75 0.8 scale

/lnw1 1 def /lnw2 2 def

newpath 0 200 moveto 990 200 lineto lnw1 setlinewidth stroke

/Times-Roman findfont 20 scalefont setfont

-15 180 moveto (0) show

/xx0 0 def /xx1 0 def /xx2 0 def /eps 0 def

/largB 12 def /zxx0 0 def /zxx1 largB def /zxx2 100 def

/baseH 200 def /deplH 150 def /haut 0 def /nHaut 0 def

/haut baseH deplH add def /nHaut baseH deplH sub def

% trace fonction

/trFct {

/xx0 zxx0 eps add def /xx1 zxx1 eps add def /xx2 zxx2 eps add def

xx0 baseH moveto xx0 haut lineto lnw1 setlinewidth stroke

xx0 haut moveto xx1 haut lineto lnw2 setlinewidth stroke

xx1 haut moveto xx1 baseH lineto lnw1 setlinewidth stroke

xx2 baseH moveto xx2 nHaut lineto stroke

xx2 nHaut moveto xx2 largB add nHaut lnw2 setlinewidth lineto stroke

xx2 largB add nHaut moveto xx2 largB add baseH

lnw1 setlinewidth lineto stroke

zxx0 200 add  baseH 10 add moveto zxx0 200 add baseH lineto stroke

} def

% Fin trace fonction

% trace fonction2

/trFct2 {

/xx0 zxx0 eps add def /xx1 zxx1 eps add def /xx2 zxx2 eps add def

xx0 baseH moveto xx0 haut lineto lnw1 setlinewidth stroke

xx0 haut moveto xx1 haut lineto lnw2 setlinewidth stroke

xx1 haut moveto xx1 baseH lineto lnw1 setlinewidth stroke

xx2 baseH moveto xx2 nHaut lineto stroke

xx2 nHaut moveto xx2 largB add nHaut lineto lnw2 setlinewidth stroke

xx2 largB add nHaut moveto xx2 largB add baseH

lnw1 setlinewidth lineto stroke

} def

/repTrfct { /zxx0i zxx0 def /zxx1i zxx1 def

/zxx2i zxx2 def

/trsl 25 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/lnw1 0.3 def /lnw2 0.6 def trFct2

/zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def trFct2

/zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def trFct2

/lnw1 1 def /lnw2 2 def

/zxx0 zxx0i def /zxx1 zxx1i def

/zxx2 zxx2i def } def


% Fin trace fonction2

% write symb

/char1 (a) def /char2 (a) def

/wrSymb {/Times-Roman findfont 20 scalefont setfont

xx0 2 sub baseH 20 sub moveto (n) show

xx0 6 add baseH 30 sub moveto char1 show

/Symbol findfont 20 scalefont setfont

xx0 12 add  baseH 20 sub moveto char2 show

/Times-Roman findfont 20 scalefont setfont } def

% Fin write symb

/eps 0 def trFct

/Symbol findfont 20 scalefont setfont

zxx1 10 sub baseH 20 sub moveto (e) show

zxx1 2 sub baseH 32 sub moveto (1/2)show

zxx2 12 add baseH 20 sub moveto (e) show

zxx2 18 add  baseH 32 sub moveto (b)show

repTrfct

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/Times-Roman findfont 20 scalefont setfont

/eps -6 def trFct

/char1 (1) def /char2 (a) def wrSymb

zxx0 10 sub  baseH 20 add moveto (1/q) show

repTrfct

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/eps 10 def trFct

zxx0 10 sub baseH 20 add moveto (2/q) show

/char1 (2) def /char2 (a) def wrSymb

repTrfct

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

/eps -6 def trFct

/char1 (3) def /char2 (a) def wrSymb

zxx0 10 sub baseH 20 add moveto (3/q) show

repTrfct

/trsl 200 def /zxx0 zxx0 trsl add def

/zxx1 zxx1 trsl add def /zxx2 zxx2 trsl add def

zxx0 10 sub baseH 20 add moveto (4/q) show

/eps 5 def trFct2

/char1 (4) def /char2 (a) def wrSymb

repTrfct

copypage


==> bill-fig7.tex <==
%%BoundingBox: 85 420 500 490
newpath 0.4 setlinewidth /l { lineto } def /m { moveto } def -90.879
179.852 m -90.879 179.852 l -90.879 179.852 m -62.621 179.852 l
-62.621 179.852 m -62.621 200.148 l -62.621 200.148 m -62.621
200.148 l -62.621 200.148 m -90.879 200.148 l -90.879 200.148 m
-90.879 200.148 l -90.879 200.148 m -90.879 179.852 l -20.129
179.852 m -20.129 179.852 l -20.129 179.852 m 8.129 179.852 l 8.129
179.852 m 8.129 200.148 l 8.129 200.148 m 8.129 200.148 l 8.129
200.148 m -20.129 200.148 l -20.129 200.148 m -20.129 200.148 l
-20.129 200.148 m -20.129 179.852 l 50.621 179.852 m 50.621 179.852
l 50.621 179.852 m 78.879 179.852 l 78.879 179.852 m 78.879 200.148
l 78.879 200.148 m 78.879 200.148 l 78.879 200.148 m 50.621 200.148
l 50.621 200.148 m 50.621 200.148 l 50.621 200.148 m 50.621 179.852
l 121.371 179.852 m 121.371 179.852 l 121.371 179.852 m 149.629
179.852 l 149.629 179.852 m 149.629 200.148 l 149.629 200.148 m
149.629 200.148 l 149.629 200.148 m 121.371 200.148 l 121.371
200.148 m 121.371 200.148 l 121.371 200.148 m 121.371 179.852 l
192.121 179.852 m 192.121 179.852 l 192.121 179.852 m 220.379
179.852 l 220.379 179.852 m 220.379 200.148 l 220.379 200.148 m
220.379 200.148 l 220.379 200.148 m 192.121 200.148 l 192.121
200.148 m 192.121 200.148 l 192.121 200.148 m 192.121 179.852 l
262.871 179.852 m 262.871 179.852 l 262.871 179.852 m 291.129
179.852 l 291.129 179.852 m 291.129 200.148 l 291.129 200.148 m
291.129 200.148 l 291.129 200.148 m 262.871 200.148 l 262.871
200.148 m 262.871 200.148 l 262.871 200.148 m 262.871 179.852 l
333.621 179.852 m 333.621 179.852 l 333.621 179.852 m 361.879
179.852 l 361.879 179.852 m 361.879 200.148 l 361.879 200.148 m
361.879 200.148 l 361.879 200.148 m 333.621 200.148 l 333.621
200.148 m 333.621 200.148 l 333.621 200.148 m 333.621 179.852 l
404.371 179.852 m 404.371 179.852 l 404.371 179.852 m 432.629
179.852 l 432.629 179.852 m 432.629 200.148 l 432.629 200.148 m
432.629 200.148 l 432.629 200.148 m 404.371 200.148 l 404.371
200.148 m 404.371 200.148 l 404.371 200.148 m 404.371 179.852 l
475.121 179.852 m 475.121 179.852 l 475.121 179.852 m 503.379
179.852 l 503.379 179.852 m 503.379 200.148 l 503.379 200.148 m
503.379 200.148 l 503.379 200.148 m 475.121 200.148 l 475.121
200.148 m 475.121 200.148 l 475.121 200.148 m 475.121 179.852 l
545.871 179.852 m 545.871 179.852 l 545.871 179.852 m 574.129
179.852 l 574.129 179.852 m 574.129 200.148 l 574.129 200.148 m
574.129 200.148 l 574.129 200.148 m 545.871 200.148 l 545.871
200.148 m 545.871 200.148 l 545.871 200.148 m 545.871 179.852 l
616.621 179.852 m 616.621 179.852 l 616.621 179.852 m 644.879
179.852 l 644.879 179.852 m 644.879 200.148 l 644.879 200.148 m
644.879 200.148 l 644.879 200.148 m 616.621 200.148 l 616.621
200.148 m 616.621 200.148 l 616.621 200.148 m 616.621 179.852 l
-90.879 217.052 m -90.879 217.052 l -90.879 217.052 m -62.621
217.052 l -62.621 217.052 m -62.621 237.348 l -62.621 237.348 m
-62.621 237.348 l -62.621 237.348 m -90.879 237.348 l -90.879
237.348 m -90.879 237.348 l -90.879 237.348 m -90.879 217.052 l
-20.129 217.052 m -20.129 217.052 l -20.129 217.052 m 8.129 217.052
l 8.129 217.052 m 8.129 237.348 l 8.129 237.348 m 8.129 237.348 l
8.129 237.348 m -20.129 237.348 l -20.129 237.348 m -20.129 237.348
l -20.129 237.348 m -20.129 217.052 l 50.621 217.052 m 50.621
217.052 l 50.621 217.052 m 78.879 217.052 l 78.879 217.052 m 78.879
237.348 l 78.879 237.348 m 78.879 237.348 l 78.879 237.348 m 50.621
237.348 l 50.621 237.348 m 50.621 237.348 l 50.621 237.348 m 50.621
217.052 l 121.371 217.052 m 121.371 217.052 l 121.371 217.052 m
149.629 217.052 l 149.629 217.052 m 149.629 237.348 l 149.629
237.348 m 149.629 237.348 l 149.629 237.348 m 121.371 237.348 l
121.371 237.348 m 121.371 237.348 l 121.371 237.348 m 121.371
217.052 l 192.121 217.052 m 192.121 217.052 l 192.121 217.052 m
220.379 217.052 l 220.379 217.052 m 220.379 237.348 l 220.379
237.348 m 220.379 237.348 l 220.379 237.348 m 192.121 237.348 l
192.121 237.348 m 192.121 237.348 l 192.121 237.348 m 192.121
217.052 l 262.871 217.052 m 262.871 217.052 l 262.871 217.052 m
291.129 217.052 l 291.129 217.052 m 291.129 237.348 l 291.129
237.348 m 291.129 237.348 l 291.129 237.348 m 262.871 237.348 l
262.871 237.348 m 262.871 237.348 l 262.871 237.348 m 262.871
217.052 l 333.621 217.052 m 333.621 217.052 l 333.621 217.052 m
361.879 217.052 l 361.879 217.052 m 361.879 237.348 l 361.879
237.348 m 361.879 237.348 l 361.879 237.348 m 333.621 237.348 l
333.621 237.348 m 333.621 237.348 l 333.621 237.348 m 333.621
217.052 l 404.371 217.052 m 404.371 217.052 l 404.371 217.052 m
432.629 217.052 l 432.629 217.052 m 432.629 237.348 l 432.629
237.348 m 432.629 237.348 l 432.629 237.348 m 404.371 237.348 l
404.371 237.348 m 404.371 237.348 l 404.371 237.348 m 404.371
217.052 l 475.121 217.052 m 475.121 217.052 l 475.121 217.052 m
503.379 217.052 l 503.379 217.052 m 503.379 237.348 l 503.379
237.348 m 503.379 237.348 l 503.379 237.348 m 475.121 237.348 l
475.121 237.348 m 475.121 237.348 l 475.121 237.348 m 475.121
217.052 l 545.871 217.052 m 545.871 217.052 l 545.871 217.052 m
574.129 217.052 l 574.129 217.052 m 574.129 237.348 l 574.129
237.348 m 574.129 237.348 l 574.129 237.348 m 545.871 237.348 l
545.871 237.348 m 545.871 237.348 l 545.871 237.348 m 545.871
217.052 l 616.621 217.052 m 616.621 217.052 l 616.621 217.052 m
644.879 217.052 l 644.879 217.052 m 644.879 237.348 l 644.879
237.348 m 644.879 237.348 l 644.879 237.348 m 616.621 237.348 l
616.621 237.348 m 616.621 237.348 l 616.621 237.348 m 616.621
217.052 l -90.879 254.252 m -90.879 254.252 l -90.879 254.252 m
-62.621 254.252 l -62.621 254.252 m -62.621 274.548 l -62.621
274.548 m -62.621 274.548 l -62.621 274.548 m -90.879 274.548 l
-90.879 274.548 m -90.879 274.548 l -90.879 274.548 m -90.879
254.252 l -20.129 254.252 m -20.129 254.252 l -20.129 254.252 m
8.129 254.252 l 8.129 254.252 m 8.129 274.548 l 8.129 274.548 m
8.129 274.548 l 8.129 274.548 m -20.129 274.548 l -20.129 274.548 m
-20.129 274.548 l -20.129 274.548 m -20.129 254.252 l 50.621 254.252
m 50.621 254.252 l 50.621 254.252 m 78.879 254.252 l 78.879 254.252
m 78.879 274.548 l 78.879 274.548 m 78.879 274.548 l 78.879 274.548
m 50.621 274.548 l 50.621 274.548 m 50.621 274.548 l 50.621 274.548
m 50.621 254.252 l 121.371 254.252 m 121.371 254.252 l 121.371
254.252 m 149.629 254.252 l 149.629 254.252 m 149.629 274.548 l
149.629 274.548 m 149.629 274.548 l 149.629 274.548 m 121.371
274.548 l 121.371 274.548 m 121.371 274.548 l 121.371 274.548 m
121.371 254.252 l 192.121 254.252 m 192.121 254.252 l 192.121
254.252 m 220.379 254.252 l 220.379 254.252 m 220.379 274.548 l
220.379 274.548 m 220.379 274.548 l 220.379 274.548 m 192.121
274.548 l 192.121 274.548 m 192.121 274.548 l 192.121 274.548 m
192.121 254.252 l 262.871 254.252 m 262.871 254.252 l 262.871
254.252 m 291.129 254.252 l 291.129 254.252 m 291.129 274.548 l
291.129 274.548 m 291.129 274.548 l 291.129 274.548 m 262.871
274.548 l 262.871 274.548 m 262.871 274.548 l 262.871 274.548 m
262.871 254.252 l 333.621 254.252 m 333.621 254.252 l 333.621
254.252 m 361.879 254.252 l 361.879 254.252 m 361.879 274.548 l
361.879 274.548 m 361.879 274.548 l 361.879 274.548 m 333.621
274.548 l 333.621 274.548 m 333.621 274.548 l 333.621 274.548 m
333.621 254.252 l 404.371 254.252 m 404.371 254.252 l 404.371
254.252 m 432.629 254.252 l 432.629 254.252 m 432.629 274.548 l
432.629 274.548 m 432.629 274.548 l 432.629 274.548 m 404.371
274.548 l 404.371 274.548 m 404.371 274.548 l 404.371 274.548 m
404.371 254.252 l 475.121 254.252 m 475.121 254.252 l 475.121
254.252 m 503.379 254.252 l 503.379 254.252 m 503.379 274.548 l
503.379 274.548 m 503.379 274.548 l 503.379 274.548 m 475.121
274.548 l 475.121 274.548 m 475.121 274.548 l 475.121 274.548 m
475.121 254.252 l 545.871 254.252 m 545.871 254.252 l 545.871
254.252 m 574.129 254.252 l 574.129 254.252 m 574.129 274.548 l
574.129 274.548 m 574.129 274.548 l 574.129 274.548 m 545.871
274.548 l 545.871 274.548 m 545.871 274.548 l 545.871 274.548 m
545.871 254.252 l 616.621 254.252 m 616.621 254.252 l 616.621
254.252 m 644.879 254.252 l 644.879 254.252 m 644.879 274.548 l
644.879 274.548 m 644.879 274.548 l 644.879 274.548 m 616.621
274.548 l 616.621 274.548 m 616.621 274.548 l 616.621 274.548 m
616.621 254.252 l -90.879 291.452 m -90.879 291.452 l -90.879
291.452 m -62.621 291.452 l -62.621 291.452 m -62.621 311.748 l
-62.621 311.748 m -62.621 311.748 l -62.621 311.748 m -90.879
311.748 l -90.879 311.748 m -90.879 311.748 l -90.879 311.748 m
-90.879 291.452 l -20.129 291.452 m -20.129 291.452 l -20.129
291.452 m 8.129 291.452 l 8.129 291.452 m 8.129 311.748 l 8.129
311.748 m 8.129 311.748 l 8.129 311.748 m -20.129 311.748 l -20.129
311.748 m -20.129 311.748 l -20.129 311.748 m -20.129 291.452 l
50.621 291.452 m 50.621 291.452 l 50.621 291.452 m 78.879 291.452 l
78.879 291.452 m 78.879 311.748 l 78.879 311.748 m 78.879 311.748 l
78.879 311.748 m 50.621 311.748 l 50.621 311.748 m 50.621 311.748 l
stroke 50.621 311.748 m 50.621 291.452 l 121.371 291.452 m 121.371
291.452 l 121.371 291.452 m 149.629 291.452 l 149.629 291.452 m
149.629 311.748 l 149.629 311.748 m 149.629 311.748 l 149.629
311.748 m 121.371 311.748 l 121.371 311.748 m 121.371 311.748 l
121.371 311.748 m 121.371 291.452 l 192.121 291.452 m 192.121
291.452 l 192.121 291.452 m 220.379 291.452 l 220.379 291.452 m
220.379 311.748 l 220.379 311.748 m 220.379 311.748 l 220.379
311.748 m 192.121 311.748 l 192.121 311.748 m 192.121 311.748 l
192.121 311.748 m 192.121 291.452 l 262.871 291.452 m 262.871
291.452 l 262.871 291.452 m 291.129 291.452 l 291.129 291.452 m
291.129 311.748 l 291.129 311.748 m 291.129 311.748 l 291.129
311.748 m 262.871 311.748 l 262.871 311.748 m 262.871 311.748 l
262.871 311.748 m 262.871 291.452 l 333.621 291.452 m 333.621
291.452 l 333.621 291.452 m 361.879 291.452 l 361.879 291.452 m
361.879 311.748 l 361.879 311.748 m 361.879 311.748 l 361.879
311.748 m 333.621 311.748 l 333.621 311.748 m 333.621 311.748 l
333.621 311.748 m 333.621 291.452 l 404.371 291.452 m 404.371
291.452 l 404.371 291.452 m 432.629 291.452 l 432.629 291.452 m
432.629 311.748 l 432.629 311.748 m 432.629 311.748 l 432.629
311.748 m 404.371 311.748 l 404.371 311.748 m 404.371 311.748 l
404.371 311.748 m 404.371 291.452 l 475.121 291.452 m 475.121
291.452 l 475.121 291.452 m 503.379 291.452 l 503.379 291.452 m
503.379 311.748 l 503.379 311.748 m 503.379 311.748 l 503.379
311.748 m 475.121 311.748 l 475.121 311.748 m 475.121 311.748 l
475.121 311.748 m 475.121 291.452 l 545.871 291.452 m 545.871
291.452 l 545.871 291.452 m 574.129 291.452 l 574.129 291.452 m
574.129 311.748 l 574.129 311.748 m 574.129 311.748 l 574.129
311.748 m 545.871 311.748 l 545.871 311.748 m 545.871 311.748 l
545.871 311.748 m 545.871 291.452 l 616.621 291.452 m 616.621
291.452 l 616.621 291.452 m 644.879 291.452 l 644.879 291.452 m
644.879 311.748 l 644.879 311.748 m 644.879 311.748 l 644.879
311.748 m 616.621 311.748 l 616.621 311.748 m 616.621 311.748 l
616.621 311.748 m 616.621 291.452 l -90.879 328.652 m -90.879
328.652 l -90.879 328.652 m -62.621 328.652 l -62.621 328.652 m
-62.621 348.948 l -62.621 348.948 m -62.621 348.948 l -62.621
348.948 m -90.879 348.948 l -90.879 348.948 m -90.879 348.948 l
-90.879 348.948 m -90.879 328.652 l -20.129 328.652 m -20.129
328.652 l -20.129 328.652 m 8.129 328.652 l 8.129 328.652 m 8.129
348.948 l 8.129 348.948 m 8.129 348.948 l 8.129 348.948 m -20.129
348.948 l -20.129 348.948 m -20.129 348.948 l -20.129 348.948 m
-20.129 328.652 l 50.621 328.652 m 50.621 328.652 l 50.621 328.652 m
78.879 328.652 l 78.879 328.652 m 78.879 348.948 l 78.879 348.948 m
78.879 348.948 l 78.879 348.948 m 50.621 348.948 l 50.621 348.948 m
50.621 348.948 l 50.621 348.948 m 50.621 328.652 l 121.371 328.652 m
121.371 328.652 l 121.371 328.652 m 149.629 328.652 l 149.629
328.652 m 149.629 348.948 l 149.629 348.948 m 149.629 348.948 l
149.629 348.948 m 121.371 348.948 l 121.371 348.948 m 121.371
348.948 l 121.371 348.948 m 121.371 328.652 l 192.121 328.652 m
192.121 328.652 l 192.121 328.652 m 220.379 328.652 l 220.379
328.652 m 220.379 348.948 l 220.379 348.948 m 220.379 348.948 l
220.379 348.948 m 192.121 348.948 l 192.121 348.948 m 192.121
348.948 l 192.121 348.948 m 192.121 328.652 l 262.871 328.652 m
262.871 328.652 l 262.871 328.652 m 291.129 328.652 l 291.129
328.652 m 291.129 348.948 l 291.129 348.948 m 291.129 348.948 l
291.129 348.948 m 262.871 348.948 l 262.871 348.948 m 262.871
348.948 l 262.871 348.948 m 262.871 328.652 l 333.621 328.652 m
333.621 328.652 l 333.621 328.652 m 361.879 328.652 l 361.879
328.652 m 361.879 348.948 l 361.879 348.948 m 361.879 348.948 l
361.879 348.948 m 333.621 348.948 l 333.621 348.948 m 333.621
348.948 l 333.621 348.948 m 333.621 328.652 l 404.371 328.652 m
404.371 328.652 l 404.371 328.652 m 432.629 328.652 l 432.629
328.652 m 432.629 348.948 l 432.629 348.948 m 432.629 348.948 l
432.629 348.948 m 404.371 348.948 l 404.371 348.948 m 404.371
348.948 l 404.371 348.948 m 404.371 328.652 l 475.121 328.652 m
475.121 328.652 l 475.121 328.652 m 503.379 328.652 l 503.379
328.652 m 503.379 348.948 l 503.379 348.948 m 503.379 348.948 l
503.379 348.948 m 475.121 348.948 l 475.121 348.948 m 475.121
348.948 l 475.121 348.948 m 475.121 328.652 l 545.871 328.652 m
545.871 328.652 l 545.871 328.652 m 574.129 328.652 l 574.129
328.652 m 574.129 348.948 l 574.129 348.948 m 574.129 348.948 l
574.129 348.948 m 545.871 348.948 l 545.871 348.948 m 545.871
348.948 l 545.871 348.948 m 545.871 328.652 l 616.621 328.652 m
616.621 328.652 l 616.621 328.652 m 644.879 328.652 l 644.879
328.652 m 644.879 348.948 l 644.879 348.948 m 644.879 348.948 l
644.879 348.948 m 616.621 348.948 l 616.621 348.948 m 616.621
348.948 l 616.621 348.948 m 616.621 328.652 l -90.879 365.852 m
-90.879 365.852 l -90.879 365.852 m -62.621 365.852 l -62.621
365.852 m -62.621 386.148 l -62.621 386.148 m -62.621 386.148 l
-62.621 386.148 m -90.879 386.148 l -90.879 386.148 m -90.879
386.148 l -90.879 386.148 m -90.879 365.852 l -20.129 365.852 m
-20.129 365.852 l -20.129 365.852 m 8.129 365.852 l 8.129 365.852 m
8.129 386.148 l 8.129 386.148 m 8.129 386.148 l 8.129 386.148 m
-20.129 386.148 l -20.129 386.148 m -20.129 386.148 l -20.129
386.148 m -20.129 365.852 l 50.621 365.852 m 50.621 365.852 l 50.621
365.852 m 78.879 365.852 l 78.879 365.852 m 78.879 386.148 l 78.879
386.148 m 78.879 386.148 l 78.879 386.148 m 50.621 386.148 l 50.621
386.148 m 50.621 386.148 l 50.621 386.148 m 50.621 365.852 l 121.371
365.852 m 121.371 365.852 l 121.371 365.852 m 149.629 365.852 l
149.629 365.852 m 149.629 386.148 l 149.629 386.148 m 149.629
386.148 l 149.629 386.148 m 121.371 386.148 l 121.371 386.148 m
121.371 386.148 l 121.371 386.148 m 121.371 365.852 l 192.121
365.852 m 192.121 365.852 l 192.121 365.852 m 220.379 365.852 l
220.379 365.852 m 220.379 386.148 l 220.379 386.148 m 220.379
386.148 l 220.379 386.148 m 192.121 386.148 l 192.121 386.148 m
192.121 386.148 l 192.121 386.148 m 192.121 365.852 l 262.871
365.852 m 262.871 365.852 l 262.871 365.852 m 291.129 365.852 l
291.129 365.852 m 291.129 386.148 l 291.129 386.148 m 291.129
386.148 l 291.129 386.148 m 262.871 386.148 l 262.871 386.148 m
262.871 386.148 l 262.871 386.148 m 262.871 365.852 l 333.621
365.852 m 333.621 365.852 l 333.621 365.852 m 361.879 365.852 l
361.879 365.852 m 361.879 386.148 l 361.879 386.148 m 361.879
386.148 l 361.879 386.148 m 333.621 386.148 l 333.621 386.148 m
333.621 386.148 l 333.621 386.148 m 333.621 365.852 l 404.371
365.852 m 404.371 365.852 l 404.371 365.852 m 432.629 365.852 l
432.629 365.852 m 432.629 386.148 l 432.629 386.148 m 432.629
386.148 l 432.629 386.148 m 404.371 386.148 l 404.371 386.148 m
404.371 386.148 l 404.371 386.148 m 404.371 365.852 l 475.121
365.852 m 475.121 365.852 l 475.121 365.852 m 503.379 365.852 l
503.379 365.852 m 503.379 386.148 l 503.379 386.148 m 503.379
386.148 l 503.379 386.148 m 475.121 386.148 l 475.121 386.148 m
475.121 386.148 l 475.121 386.148 m 475.121 365.852 l 545.871
365.852 m 545.871 365.852 l 545.871 365.852 m 574.129 365.852 l
574.129 365.852 m 574.129 386.148 l 574.129 386.148 m 574.129
386.148 l 574.129 386.148 m 545.871 386.148 l 545.871 386.148 m
545.871 386.148 l 545.871 386.148 m 545.871 365.852 l 616.621
365.852 m 616.621 365.852 l 616.621 365.852 m 644.879 365.852 l
644.879 365.852 m 644.879 386.148 l 644.879 386.148 m 644.879
386.148 l 644.879 386.148 m 616.621 386.148 l 616.621 386.148 m
616.621 386.148 l 616.621 386.148 m 616.621 365.852 l -90.879
403.052 m -90.879 403.052 l -90.879 403.052 m -62.621 403.052 l
-62.621 403.052 m -62.621 423.348 l -62.621 423.348 m -62.621
423.348 l -62.621 423.348 m -90.879 423.348 l -90.879 423.348 m
-90.879 423.348 l -90.879 423.348 m -90.879 403.052 l -20.129
403.052 m -20.129 403.052 l -20.129 403.052 m 8.129 403.052 l 8.129
403.052 m 8.129 423.348 l 8.129 423.348 m 8.129 423.348 l 8.129
423.348 m -20.129 423.348 l -20.129 423.348 m -20.129 423.348 l
-20.129 423.348 m -20.129 403.052 l 50.621 403.052 m 50.621 403.052
l 50.621 403.052 m 78.879 403.052 l 78.879 403.052 m 78.879 423.348
l 78.879 423.348 m 78.879 423.348 l 78.879 423.348 m 50.621 423.348
l 50.621 423.348 m 50.621 423.348 l 50.621 423.348 m 50.621 403.052
l 121.371 403.052 m 121.371 403.052 l 121.371 403.052 m 149.629
403.052 l 149.629 403.052 m 149.629 423.348 l 149.629 423.348 m
149.629 423.348 l 149.629 423.348 m 121.371 423.348 l 121.371
423.348 m 121.371 423.348 l 121.371 423.348 m 121.371 403.052 l
192.121 403.052 m 192.121 403.052 l 192.121 403.052 m 220.379
403.052 l 220.379 403.052 m 220.379 423.348 l 220.379 423.348 m
220.379 423.348 l 220.379 423.348 m 192.121 423.348 l 192.121
423.348 m 192.121 423.348 l 192.121 423.348 m 192.121 403.052 l
262.871 403.052 m 262.871 403.052 l 262.871 403.052 m 291.129
403.052 l 291.129 403.052 m 291.129 423.348 l 291.129 423.348 m
291.129 423.348 l 291.129 423.348 m 262.871 423.348 l stroke 262.871
423.348 m 262.871 423.348 l 262.871 423.348 m 262.871 403.052 l
333.621 403.052 m 333.621 403.052 l 333.621 403.052 m 361.879
403.052 l 361.879 403.052 m 361.879 423.348 l 361.879 423.348 m
361.879 423.348 l 361.879 423.348 m 333.621 423.348 l 333.621
423.348 m 333.621 423.348 l 333.621 423.348 m 333.621 403.052 l
404.371 403.052 m 404.371 403.052 l 404.371 403.052 m 432.629
403.052 l 432.629 403.052 m 432.629 423.348 l 432.629 423.348 m
432.629 423.348 l 432.629 423.348 m 404.371 423.348 l 404.371
423.348 m 404.371 423.348 l 404.371 423.348 m 404.371 403.052 l
475.121 403.052 m 475.121 403.052 l 475.121 403.052 m 503.379
403.052 l 503.379 403.052 m 503.379 423.348 l 503.379 423.348 m
503.379 423.348 l 503.379 423.348 m 475.121 423.348 l 475.121
423.348 m 475.121 423.348 l 475.121 423.348 m 475.121 403.052 l
545.871 403.052 m 545.871 403.052 l 545.871 403.052 m 574.129
403.052 l 574.129 403.052 m 574.129 423.348 l 574.129 423.348 m
574.129 423.348 l 574.129 423.348 m 545.871 423.348 l 545.871
423.348 m 545.871 423.348 l 545.871 423.348 m 545.871 403.052 l
616.621 403.052 m 616.621 403.052 l 616.621 403.052 m 644.879
403.052 l 644.879 403.052 m 644.879 423.348 l 644.879 423.348 m
644.879 423.348 l 644.879 423.348 m 616.621 423.348 l 616.621
423.348 m 616.621 423.348 l 616.621 423.348 m 616.621 403.052 l
-90.879 440.252 m -90.879 440.252 l -90.879 440.252 m -62.621
440.252 l -62.621 440.252 m -62.621 460.548 l -62.621 460.548 m
-62.621 460.548 l -62.621 460.548 m -90.879 460.548 l -90.879
460.548 m -90.879 460.548 l -90.879 460.548 m -90.879 440.252 l
-20.129 440.252 m -20.129 440.252 l -20.129 440.252 m 8.129 440.252
l 8.129 440.252 m 8.129 460.548 l 8.129 460.548 m 8.129 460.548 l
8.129 460.548 m -20.129 460.548 l -20.129 460.548 m -20.129 460.548
l -20.129 460.548 m -20.129 440.252 l 50.621 440.252 m 50.621
440.252 l 50.621 440.252 m 78.879 440.252 l 78.879 440.252 m 78.879
460.548 l 78.879 460.548 m 78.879 460.548 l 78.879 460.548 m 50.621
460.548 l 50.621 460.548 m 50.621 460.548 l 50.621 460.548 m 50.621
440.252 l 121.371 440.252 m 121.371 440.252 l 121.371 440.252 m
149.629 440.252 l 149.629 440.252 m 149.629 460.548 l 149.629
460.548 m 149.629 460.548 l 149.629 460.548 m 121.371 460.548 l
121.371 460.548 m 121.371 460.548 l 121.371 460.548 m 121.371
440.252 l 192.121 440.252 m 192.121 440.252 l 192.121 440.252 m
220.379 440.252 l 220.379 440.252 m 220.379 460.548 l 220.379
460.548 m 220.379 460.548 l 220.379 460.548 m 192.121 460.548 l
192.121 460.548 m 192.121 460.548 l 192.121 460.548 m 192.121
440.252 l 262.871 440.252 m 262.871 440.252 l 262.871 440.252 m
291.129 440.252 l 291.129 440.252 m 291.129 460.548 l 291.129
460.548 m 291.129 460.548 l 291.129 460.548 m 262.871 460.548 l
262.871 460.548 m 262.871 460.548 l 262.871 460.548 m 262.871
440.252 l 333.621 440.252 m 333.621 440.252 l 333.621 440.252 m
361.879 440.252 l 361.879 440.252 m 361.879 460.548 l 361.879
460.548 m 361.879 460.548 l 361.879 460.548 m 333.621 460.548 l
333.621 460.548 m 333.621 460.548 l 333.621 460.548 m 333.621
440.252 l 404.371 440.252 m 404.371 440.252 l 404.371 440.252 m
432.629 440.252 l 432.629 440.252 m 432.629 460.548 l 432.629
460.548 m 432.629 460.548 l 432.629 460.548 m 404.371 460.548 l
404.371 460.548 m 404.371 460.548 l 404.371 460.548 m 404.371
440.252 l 475.121 440.252 m 475.121 440.252 l 475.121 440.252 m
503.379 440.252 l 503.379 440.252 m 503.379 460.548 l 503.379
460.548 m 503.379 460.548 l 503.379 460.548 m 475.121 460.548 l
475.121 460.548 m 475.121 460.548 l 475.121 460.548 m 475.121
440.252 l 545.871 440.252 m 545.871 440.252 l 545.871 440.252 m
574.129 440.252 l 574.129 440.252 m 574.129 460.548 l 574.129
460.548 m 574.129 460.548 l 574.129 460.548 m 545.871 460.548 l
545.871 460.548 m 545.871 460.548 l 545.871 460.548 m 545.871
440.252 l 616.621 440.252 m 616.621 440.252 l 616.621 440.252 m
644.879 440.252 l 644.879 440.252 m 644.879 460.548 l 644.879
460.548 m 644.879 460.548 l 644.879 460.548 m 616.621 460.548 l
616.621 460.548 m 616.621 460.548 l 616.621 460.548 m 616.621
440.252 l -90.879 477.452 m -90.879 477.452 l -90.879 477.452 m
-62.621 477.452 l -62.621 477.452 m -62.621 497.748 l -62.621
497.748 m -62.621 497.748 l -62.621 497.748 m -90.879 497.748 l
-90.879 497.748 m -90.879 497.748 l -90.879 497.748 m -90.879
477.452 l -20.129 477.452 m -20.129 477.452 l -20.129 477.452 m
8.129 477.452 l 8.129 477.452 m 8.129 497.748 l 8.129 497.748 m
8.129 497.748 l 8.129 497.748 m -20.129 497.748 l -20.129 497.748 m
-20.129 497.748 l -20.129 497.748 m -20.129 477.452 l 50.621 477.452
m 50.621 477.452 l 50.621 477.452 m 78.879 477.452 l 78.879 477.452
m 78.879 497.748 l 78.879 497.748 m 78.879 497.748 l 78.879 497.748
m 50.621 497.748 l 50.621 497.748 m 50.621 497.748 l 50.621 497.748
m 50.621 477.452 l 121.371 477.452 m 121.371 477.452 l 121.371
477.452 m 149.629 477.452 l 149.629 477.452 m 149.629 497.748 l
149.629 497.748 m 149.629 497.748 l 149.629 497.748 m 121.371
497.748 l 121.371 497.748 m 121.371 497.748 l 121.371 497.748 m
121.371 477.452 l 192.121 477.452 m 192.121 477.452 l 192.121
477.452 m 220.379 477.452 l 220.379 477.452 m 220.379 497.748 l
220.379 497.748 m 220.379 497.748 l 220.379 497.748 m 192.121
497.748 l 192.121 497.748 m 192.121 497.748 l 192.121 497.748 m
192.121 477.452 l 262.871 477.452 m 262.871 477.452 l 262.871
477.452 m 291.129 477.452 l 291.129 477.452 m 291.129 497.748 l
291.129 497.748 m 291.129 497.748 l 291.129 497.748 m 262.871
497.748 l 262.871 497.748 m 262.871 497.748 l 262.871 497.748 m
262.871 477.452 l 333.621 477.452 m 333.621 477.452 l 333.621
477.452 m 361.879 477.452 l 361.879 477.452 m 361.879 497.748 l
361.879 497.748 m 361.879 497.748 l 361.879 497.748 m 333.621
497.748 l 333.621 497.748 m 333.621 497.748 l 333.621 497.748 m
333.621 477.452 l 404.371 477.452 m 404.371 477.452 l 404.371
477.452 m 432.629 477.452 l 432.629 477.452 m 432.629 497.748 l
432.629 497.748 m 432.629 497.748 l 432.629 497.748 m 404.371
497.748 l 404.371 497.748 m 404.371 497.748 l 404.371 497.748 m
404.371 477.452 l 475.121 477.452 m 475.121 477.452 l 475.121
477.452 m 503.379 477.452 l 503.379 477.452 m 503.379 497.748 l
503.379 497.748 m 503.379 497.748 l 503.379 497.748 m 475.121
497.748 l 475.121 497.748 m 475.121 497.748 l 475.121 497.748 m
475.121 477.452 l 545.871 477.452 m 545.871 477.452 l 545.871
477.452 m 574.129 477.452 l 574.129 477.452 m 574.129 497.748 l
574.129 497.748 m 574.129 497.748 l 574.129 497.748 m 545.871
497.748 l 545.871 497.748 m 545.871 497.748 l 545.871 497.748 m
545.871 477.452 l 616.621 477.452 m 616.621 477.452 l 616.621
477.452 m 644.879 477.452 l 644.879 477.452 m 644.879 497.748 l
644.879 497.748 m 644.879 497.748 l 644.879 497.748 m 616.621
497.748 l 616.621 497.748 m 616.621 497.748 l 616.621 497.748 m
616.621 477.452 l -90.879 514.652 m -90.879 514.652 l -90.879
514.652 m -62.621 514.652 l -62.621 514.652 m -62.621 534.948 l
-62.621 534.948 m -62.621 534.948 l -62.621 534.948 m -90.879
534.948 l -90.879 534.948 m -90.879 534.948 l -90.879 534.948 m
-90.879 514.652 l -20.129 514.652 m -20.129 514.652 l -20.129
514.652 m 8.129 514.652 l 8.129 514.652 m 8.129 534.948 l 8.129
534.948 m 8.129 534.948 l 8.129 534.948 m -20.129 534.948 l -20.129
534.948 m -20.129 534.948 l -20.129 534.948 m -20.129 514.652 l
50.621 514.652 m 50.621 514.652 l 50.621 514.652 m 78.879 514.652 l
78.879 514.652 m 78.879 534.948 l 78.879 534.948 m 78.879 534.948 l
78.879 534.948 m 50.621 534.948 l 50.621 534.948 m 50.621 534.948 l
50.621 534.948 m 50.621 514.652 l 121.371 514.652 m 121.371 514.652
l 121.371 514.652 m 149.629 514.652 l 149.629 514.652 m 149.629
534.948 l 149.629 534.948 m 149.629 534.948 l 149.629 534.948 m
121.371 534.948 l 121.371 534.948 m 121.371 534.948 l 121.371
534.948 m 121.371 514.652 l 192.121 514.652 m 192.121 514.652 l
192.121 514.652 m 220.379 514.652 l 220.379 514.652 m 220.379
534.948 l 220.379 534.948 m 220.379 534.948 l 220.379 534.948 m
192.121 534.948 l 192.121 534.948 m 192.121 534.948 l 192.121
534.948 m 192.121 514.652 l 262.871 514.652 m 262.871 514.652 l
262.871 514.652 m 291.129 514.652 l 291.129 514.652 m 291.129
534.948 l 291.129 534.948 m 291.129 534.948 l 291.129 534.948 m
262.871 534.948 l 262.871 534.948 m 262.871 534.948 l 262.871
534.948 m 262.871 514.652 l 333.621 514.652 m 333.621 514.652 l
333.621 514.652 m 361.879 514.652 l 361.879 514.652 m 361.879
534.948 l 361.879 534.948 m 361.879 534.948 l 361.879 534.948 m
333.621 534.948 l 333.621 534.948 m 333.621 534.948 l 333.621
534.948 m 333.621 514.652 l 404.371 514.652 m 404.371 514.652 l
404.371 514.652 m 432.629 514.652 l 432.629 514.652 m 432.629
534.948 l 432.629 534.948 m 432.629 534.948 l 432.629 534.948 m
404.371 534.948 l 404.371 534.948 m 404.371 534.948 l 404.371
534.948 m 404.371 514.652 l 475.121 514.652 m 475.121 514.652 l
475.121 514.652 m 503.379 514.652 l 503.379 514.652 m 503.379
534.948 l 503.379 534.948 m 503.379 534.948 l stroke 503.379 534.948
m 475.121 534.948 l 475.121 534.948 m 475.121 534.948 l 475.121
534.948 m 475.121 514.652 l 545.871 514.652 m 545.871 514.652 l
545.871 514.652 m 574.129 514.652 l 574.129 514.652 m 574.129
534.948 l 574.129 534.948 m 574.129 534.948 l 574.129 534.948 m
545.871 534.948 l 545.871 534.948 m 545.871 534.948 l 545.871
534.948 m 545.871 514.652 l 616.621 514.652 m 616.621 514.652 l
616.621 514.652 m 644.879 514.652 l 644.879 514.652 m 644.879
534.948 l 644.879 534.948 m 644.879 534.948 l 644.879 534.948 m
616.621 534.948 l 616.621 534.948 m 616.621 534.948 l 616.621
534.948 m 616.621 514.652 l -90.879 551.852 m -90.879 551.852 l
-90.879 551.852 m -62.621 551.852 l -62.621 551.852 m -62.621
572.148 l -62.621 572.148 m -62.621 572.148 l -62.621 572.148 m
-90.879 572.148 l -90.879 572.148 m -90.879 572.148 l -90.879
572.148 m -90.879 551.852 l -20.129 551.852 m -20.129 551.852 l
-20.129 551.852 m 8.129 551.852 l 8.129 551.852 m 8.129 572.148 l
8.129 572.148 m 8.129 572.148 l 8.129 572.148 m -20.129 572.148 l
-20.129 572.148 m -20.129 572.148 l -20.129 572.148 m -20.129
551.852 l 50.621 551.852 m 50.621 551.852 l 50.621 551.852 m 78.879
551.852 l 78.879 551.852 m 78.879 572.148 l 78.879 572.148 m 78.879
572.148 l 78.879 572.148 m 50.621 572.148 l 50.621 572.148 m 50.621
572.148 l 50.621 572.148 m 50.621 551.852 l 121.371 551.852 m
121.371 551.852 l 121.371 551.852 m 149.629 551.852 l 149.629
551.852 m 149.629 572.148 l 149.629 572.148 m 149.629 572.148 l
149.629 572.148 m 121.371 572.148 l 121.371 572.148 m 121.371
572.148 l 121.371 572.148 m 121.371 551.852 l 192.121 551.852 m
192.121 551.852 l 192.121 551.852 m 220.379 551.852 l 220.379
551.852 m 220.379 572.148 l 220.379 572.148 m 220.379 572.148 l
220.379 572.148 m 192.121 572.148 l 192.121 572.148 m 192.121
572.148 l 192.121 572.148 m 192.121 551.852 l 262.871 551.852 m
262.871 551.852 l 262.871 551.852 m 291.129 551.852 l 291.129
551.852 m 291.129 572.148 l 291.129 572.148 m 291.129 572.148 l
291.129 572.148 m 262.871 572.148 l 262.871 572.148 m 262.871
572.148 l 262.871 572.148 m 262.871 551.852 l 333.621 551.852 m
333.621 551.852 l 333.621 551.852 m 361.879 551.852 l 361.879
551.852 m 361.879 572.148 l 361.879 572.148 m 361.879 572.148 l
361.879 572.148 m 333.621 572.148 l 333.621 572.148 m 333.621
572.148 l 333.621 572.148 m 333.621 551.852 l 404.371 551.852 m
404.371 551.852 l 404.371 551.852 m 432.629 551.852 l 432.629
551.852 m 432.629 572.148 l 432.629 572.148 m 432.629 572.148 l
432.629 572.148 m 404.371 572.148 l 404.371 572.148 m 404.371
572.148 l 404.371 572.148 m 404.371 551.852 l 475.121 551.852 m
475.121 551.852 l 475.121 551.852 m 503.379 551.852 l 503.379
551.852 m 503.379 572.148 l 503.379 572.148 m 503.379 572.148 l
503.379 572.148 m 475.121 572.148 l 475.121 572.148 m 475.121
572.148 l 475.121 572.148 m 475.121 551.852 l 545.871 551.852 m
545.871 551.852 l 545.871 551.852 m 574.129 551.852 l 574.129
551.852 m 574.129 572.148 l 574.129 572.148 m 574.129 572.148 l
574.129 572.148 m 545.871 572.148 l 545.871 572.148 m 545.871
572.148 l 545.871 572.148 m 545.871 551.852 l 616.621 551.852 m
616.621 551.852 l 616.621 551.852 m 644.879 551.852 l 644.879
551.852 m 644.879 572.148 l 644.879 572.148 m 644.879 572.148 l
644.879 572.148 m 616.621 572.148 l 616.621 572.148 m 616.621
572.148 l 616.621 572.148 m 616.621 551.852 l 277.000 376.000 m
277.000 376.000 l 291.129 384.532 m 291.129 384.532 l 291.129
384.532 m 291.129 384.532 l 291.129 384.532 m 333.621 406.874 l
333.621 406.874 m 333.621 406.874 l 333.621 406.874 m 333.621
406.874 l 333.621 406.874 m 270.141 440.252 l 270.141 440.252 m
270.141 440.252 l 270.141 440.252 m 270.141 440.252 l 270.141
440.252 m 220.379 414.087 l 220.379 414.087 m 220.379 414.087 l
220.379 414.087 m 220.379 414.087 l 220.379 414.087 m 273.516
386.148 l 273.516 386.148 m 273.516 386.148 l 273.516 386.148 m
273.516 386.148 l 273.516 386.148 m 333.621 417.751 l 333.621
417.751 m 333.621 417.751 l 333.621 417.751 m 333.621 417.751 l
333.621 417.751 m 290.827 440.252 l 290.827 440.252 m 290.827
440.252 l 290.827 440.252 m 290.827 440.252 l 290.827 440.252 m
220.379 403.211 l 220.379 403.211 m 220.379 403.211 l 220.379
403.211 m 220.379 403.211 l 220.379 403.211 m 262.871 380.868 l
262.871 380.868 m 262.871 380.868 l 262.871 380.868 m 262.871
380.868 l 262.871 380.868 m 202.162 348.948 l 202.162 348.948 m
202.162 348.948 l 202.162 348.948 m 202.162 348.948 l 202.162
348.948 m 149.629 376.570 l 149.629 376.570 m 149.629 376.570 l
149.629 376.570 m 149.629 376.570 l 149.629 376.570 m 199.995
403.052 l 199.995 403.052 m 199.995 403.052 l 199.995 403.052 m
199.995 403.052 l 199.995 403.052 m 262.871 369.992 l 262.871
369.992 m 262.871 369.992 l 262.871 369.992 m 262.871 369.992 l
262.871 369.992 m 220.379 347.650 l 220.379 347.650 m 220.379
347.650 l 220.379 347.650 m 220.379 347.650 l 220.379 347.650 m
288.659 311.748 l 288.659 311.748 m 288.659 311.748 l 288.659
311.748 m 288.659 311.748 l 288.659 311.748 m 333.621 335.389 l
333.621 335.389 m 333.621 335.389 l 333.621 335.389 m 333.621
335.389 l 333.621 335.389 m 275.684 365.852 l 275.684 365.852 m
275.684 365.852 l 275.684 365.852 m 275.684 365.852 l 275.684
365.852 m 220.379 336.773 l 220.379 336.773 m 220.379 336.773 l
220.379 336.773 m 220.379 336.773 l 220.379 336.773 m 267.974
311.748 l 267.974 311.748 m 267.974 311.748 l 267.974 311.748 m
267.974 311.748 l 267.974 311.748 m 333.621 346.265 l 333.621
346.265 m 333.621 346.265 l 333.621 346.265 m 333.621 346.265 l
333.621 346.265 m 291.129 368.608 l 291.129 368.608 m 291.129
368.608 l 291.129 368.608 m 291.129 368.608 l 291.129 368.608 m
356.638 403.052 l 356.638 403.052 m 356.638 403.052 l 356.638
403.052 m 356.638 403.052 l 356.638 403.052 m 404.371 377.954 l
404.371 377.954 m 404.371 377.954 l 404.371 377.954 m 404.371
377.954 l 404.371 377.954 m 349.205 348.948 l 349.205 348.948 m
349.205 348.948 l 349.205 348.948 m 349.205 348.948 l 349.205
348.948 m 291.129 379.484 l 291.129 379.484 m 291.129 379.484 l
291.129 379.484 m 291.129 379.484 l 291.129 379.484 m 335.952
403.052 l 335.952 403.052 m 335.952 403.052 l 335.952 403.052 m
335.952 403.052 l 335.952 403.052 m 404.371 367.078 l 404.371
367.078 m 404.371 367.078 l 404.371 367.078 m 404.371 367.078 l
404.371 367.078 m 361.879 344.735 l 361.879 344.735 m 361.879
344.735 l 361.879 344.735 m 361.879 344.735 l 361.879 344.735 m
424.617 311.748 l 424.617 311.748 m 424.617 311.748 l 424.617
311.748 m 424.617 311.748 l 424.617 311.748 m 475.121 338.303 l
475.121 338.303 m 475.121 338.303 l 475.121 338.303 m 475.121
338.303 l 475.121 338.303 m 422.726 365.852 l 422.726 365.852 m
422.726 365.852 l 422.726 365.852 m 422.726 365.852 l 422.726
365.852 m 361.879 333.859 l 361.879 333.859 m 361.879 333.859 l
361.879 333.859 m 361.879 333.859 l 361.879 333.859 m 404.371
311.516 l 404.371 311.516 m 404.371 311.516 l 404.371 311.516 m
404.371 311.516 l 404.371 311.516 m 334.062 274.548 l 334.062
274.548 m 334.062 274.548 l 334.062 274.548 m 334.062 274.548 l
334.062 274.548 m 291.129 297.122 l 291.129 297.122 m 291.129
297.122 l 291.129 297.122 m 291.129 297.122 l 291.129 297.122 m
351.095 328.652 l 351.095 328.652 m 351.095 328.652 l 351.095
328.652 m 351.095 328.652 l 351.095 328.652 m 404.371 300.640 l
404.371 300.640 m 404.371 300.640 l 404.371 300.640 m 404.371
300.640 l 404.371 300.640 m 354.748 274.548 l 354.748 274.548 m
354.748 274.548 l 354.748 274.548 m 354.748 274.548 l 354.748
274.548 m 291.129 307.998 l 291.129 307.998 m 291.129 307.998 l
291.129 307.998 m 291.129 307.998 l 291.129 307.998 m 333.621
330.341 l 333.621 330.341 m 333.621 330.341 l 333.621 330.341 m
333.621 330.341 l 333.621 330.341 m 266.083 365.852 l 266.083
365.852 m 266.083 365.852 l 266.083 365.852 m 266.083 365.852 l
266.083 365.852 m 220.379 341.821 l 220.379 341.821 m 220.379
341.821 l 220.379 341.821 m 220.379 341.821 l 220.379 341.821 m
277.574 311.748 l 277.574 311.748 m 277.574 311.748 l 277.574
311.748 m 277.574 311.748 l 277.574 311.748 m 333.621 341.217 l
333.621 341.217 m 333.621 341.217 l 333.621 341.217 m 333.621
341.217 l 333.621 341.217 m 286.769 365.852 l 286.769 365.852 m
286.769 365.852 l 286.769 365.852 m 286.769 365.852 l 286.769
365.852 m 220.379 330.944 l 220.379 330.944 m 220.379 330.944 l
220.379 330.944 m 220.379 330.944 l 220.379 330.944 m 262.871
308.602 l 262.871 308.602 m 262.871 308.602 l 262.871 308.602 m
262.871 308.602 l 262.871 308.602 m 198.105 274.548 l 198.105
274.548 m 198.105 274.548 l 198.105 274.548 m 198.105 274.548 l
198.105 274.548 m 149.629 300.036 l 149.629 300.036 m 149.629
300.036 l 149.629 300.036 m 149.629 300.036 l 149.629 300.036 m
204.053 328.652 l 204.053 328.652 m 204.053 328.652 l 204.053
328.652 m 204.053 328.652 l 204.053 328.652 m 262.871 297.725 l
262.871 297.725 m 262.871 297.725 l 262.871 297.725 m 262.871
297.725 l 262.871 297.725 m 218.790 274.548 l 218.790 274.548 m
218.790 274.548 l 218.790 274.548 m 218.790 274.548 l 218.790
274.548 m 149.629 310.913 l stroke 149.629 310.913 m 149.629 310.913
l 149.629 310.913 m 149.629 310.913 l 149.629 310.913 m 192.121
333.255 l 192.121 333.255 m 192.121 333.255 l 192.121 333.255 m
192.121 333.255 l 192.121 333.255 m 130.126 365.852 l 130.126
365.852 m 130.126 365.852 l 130.126 365.852 m 130.126 365.852 l
130.126 365.852 m 78.879 338.907 l 78.879 338.907 m 78.879 338.907 l
78.879 338.907 m 78.879 338.907 l 78.879 338.907 m 130.531 311.748 l
130.531 311.748 m 130.531 311.748 l 130.531 311.748 m 130.531
311.748 l 130.531 311.748 m 192.121 344.132 l 192.121 344.132 m
192.121 344.132 l 192.121 344.132 m 192.121 344.132 l 192.121
344.132 m 149.629 366.474 l 149.629 366.474 m 149.629 366.474 l
149.629 366.474 m 149.629 366.474 l 149.629 366.474 m 219.196
403.052 l 219.196 403.052 m 219.196 403.052 l 219.196 403.052 m
219.196 403.052 l 219.196 403.052 m 262.871 380.088 l 262.871
380.088 m 262.871 380.088 l 262.871 380.088 m 262.871 380.088 l
262.871 380.088 m 203.647 348.948 l 203.647 348.948 m 203.647
348.948 l 203.647 348.948 m 203.647 348.948 l 203.647 348.948 m
149.629 377.351 l 149.629 377.351 m 149.629 377.351 l 149.629
377.351 m 149.629 377.351 l 149.629 377.351 m 198.510 403.052 l
198.510 403.052 m 198.510 403.052 l 198.510 403.052 m 198.510
403.052 l 198.510 403.052 m 262.871 369.211 l 262.871 369.211 m
262.871 369.211 l 262.871 369.211 m 262.871 369.211 l 262.871
369.211 m 220.379 346.869 l 220.379 346.869 m 220.379 346.869 l
220.379 346.869 m 220.379 346.869 l 220.379 346.869 m 287.174
311.748 l 287.174 311.748 m 287.174 311.748 l 287.174 311.748 m
287.174 311.748 l 287.174 311.748 m 333.621 336.170 l 333.621
336.170 m 333.621 336.170 l 333.621 336.170 m 333.621 336.170 l
333.621 336.170 m 277.169 365.852 l 277.169 365.852 m 277.169
365.852 l 277.169 365.852 m 277.169 365.852 l 277.169 365.852 m
220.379 335.992 l 220.379 335.992 m 220.379 335.992 l 220.379
335.992 m 220.379 335.992 l 220.379 335.992 m 266.488 311.748 l
266.488 311.748 m 266.488 311.748 l 266.488 311.748 m 266.488
311.748 l 266.488 311.748 m 333.621 347.046 l 333.621 347.046 m
333.621 347.046 l 333.621 347.046 m 333.621 347.046 l 333.621
347.046 m 291.129 369.389 l 291.129 369.389 m 291.129 369.389 l
291.129 369.389 m 291.129 369.389 l 291.129 369.389 m 355.153
403.052 l 355.153 403.052 m 355.153 403.052 l 355.153 403.052 m
355.153 403.052 l 355.153 403.052 m 404.371 377.173 l 404.371
377.173 m 404.371 377.173 l 404.371 377.173 m 404.371 377.173 l
404.371 377.173 m 350.690 348.948 l 350.690 348.948 m 350.690
348.948 l 350.690 348.948 m 350.690 348.948 l 350.690 348.948 m
291.129 380.265 l 291.129 380.265 m 291.129 380.265 l 291.129
380.265 m 291.129 380.265 l 291.129 380.265 m 334.467 403.052 l
334.467 403.052 m 334.467 403.052 l 334.467 403.052 m 334.467
403.052 l 334.467 403.052 m 404.371 366.297 l 404.371 366.297 m
404.371 366.297 l 404.371 366.297 m 404.371 366.297 l 404.371
366.297 m 361.879 343.954 l 361.879 343.954 m 361.879 343.954 l
361.879 343.954 m 361.879 343.954 l 361.879 343.954 m 423.131
311.748 l 423.131 311.748 m 423.131 311.748 l 423.131 311.748 m
423.131 311.748 l 423.131 311.748 m 475.121 339.084 l 475.121
339.084 m 475.121 339.084 l 475.121 339.084 m 475.121 339.084 l
475.121 339.084 m 424.211 365.852 l 424.211 365.852 m 424.211
365.852 l 424.211 365.852 m 424.211 365.852 l 424.211 365.852 m
361.879 333.078 l 361.879 333.078 m 361.879 333.078 l 361.879
333.078 m 361.879 333.078 l 361.879 333.078 m 404.371 310.735 l
404.371 310.735 m 404.371 310.735 l 404.371 310.735 m 404.371
310.735 l 404.371 310.735 m 335.547 274.548 l 335.547 274.548 m
335.547 274.548 l 335.547 274.548 m 335.547 274.548 l 335.547
274.548 m 291.129 297.903 l 291.129 297.903 m 291.129 297.903 l
291.129 297.903 m 291.129 297.903 l 291.129 297.903 m 349.610
328.652 l 349.610 328.652 m 349.610 328.652 l 349.610 328.652 m
349.610 328.652 l 349.610 328.652 m 404.371 299.859 l 404.371
299.859 m 404.371 299.859 l 404.371 299.859 m 404.371 299.859 l
404.371 299.859 m 356.233 274.548 l 356.233 274.548 m 356.233
274.548 l 356.233 274.548 m 356.233 274.548 l 356.233 274.548 m
291.129 308.779 l 291.129 308.779 m 291.129 308.779 l 291.129
308.779 m 291.129 308.779 l 291.129 308.779 m 333.621 331.122 l
333.621 331.122 m 333.621 331.122 l 333.621 331.122 m 333.621
331.122 l 333.621 331.122 m 267.568 365.852 l 267.568 365.852 m
267.568 365.852 l 267.568 365.852 m 267.568 365.852 l 267.568
365.852 m 220.379 341.040 l 220.379 341.040 m 220.379 341.040 l
220.379 341.040 m 220.379 341.040 l 220.379 341.040 m 276.089
311.748 l 276.089 311.748 m 276.089 311.748 l 276.089 311.748 m
276.089 311.748 l 276.089 311.748 m 333.621 341.998 l 333.621
341.998 m 333.621 341.998 l 333.621 341.998 m 333.621 341.998 l
333.621 341.998 m 288.254 365.852 l 288.254 365.852 m 288.254
365.852 l 288.254 365.852 m 288.254 365.852 l 288.254 365.852 m
220.379 330.164 l 220.379 330.164 m 220.379 330.164 l 220.379
330.164 m 220.379 330.164 l 220.379 330.164 m 262.871 307.821 l
262.871 307.821 m 262.871 307.821 l 262.871 307.821 m 262.871
307.821 l 262.871 307.821 m 199.590 274.548 l 199.590 274.548 m
199.590 274.548 l 199.590 274.548 m 199.590 274.548 l 199.590
274.548 m 149.629 300.817 l 149.629 300.817 m 149.629 300.817 l
149.629 300.817 m 149.629 300.817 l 149.629 300.817 m 202.567
328.652 l 202.567 328.652 m 202.567 328.652 l 202.567 328.652 m
202.567 328.652 l 202.567 328.652 m 262.871 296.945 l 262.871
296.945 m 262.871 296.945 l 262.871 296.945 m 262.871 296.945 l
262.871 296.945 m 220.275 274.548 l 220.275 274.548 m 220.275
274.548 l 220.275 274.548 m 220.275 274.548 l 220.275 274.548 m
149.629 311.694 l 149.629 311.694 m 149.629 311.694 l 149.629
311.694 m 149.629 311.694 l 149.629 311.694 m 192.121 334.036 l
192.121 334.036 m 192.121 334.036 l 192.121 334.036 m 192.121
334.036 l 192.121 334.036 m 131.611 365.852 l 131.611 365.852 m
131.611 365.852 l 131.611 365.852 m 131.611 365.852 l 131.611
365.852 m 78.879 338.126 l 78.879 338.126 m 78.879 338.126 l 78.879
338.126 m 78.879 338.126 l 78.879 338.126 m 129.046 311.748 l
129.046 311.748 m 129.046 311.748 l 129.046 311.748 m 129.046
311.748 l 129.046 311.748 m 192.121 344.913 l 192.121 344.913 m
192.121 344.913 l 192.121 344.913 m 192.121 344.913 l 192.121
344.913 m 149.629 367.255 l 149.629 367.255 m 149.629 367.255 l
149.629 367.255 m 149.629 367.255 l 149.629 367.255 m 217.710
403.052 l 217.710 403.052 m 217.710 403.052 l 217.710 403.052 m
217.710 403.052 l 217.710 403.052 m 262.871 379.307 l 262.871
379.307 m 262.871 379.307 l 262.871 379.307 m 262.871 379.307 l
262.871 379.307 m 205.132 348.948 l 205.132 348.948 m 205.132
348.948 l 205.132 348.948 m 205.132 348.948 l 205.132 348.948 m
149.629 378.132 l 149.629 378.132 m 149.629 378.132 l 149.629
378.132 m 149.629 378.132 l 149.629 378.132 m 197.025 403.052 l
197.025 403.052 m 197.025 403.052 l 197.025 403.052 m 197.025
403.052 l 197.025 403.052 m 262.871 368.430 l 262.871 368.430 m
262.871 368.430 l 262.871 368.430 m 262.871 368.430 l 262.871
368.430 m 220.379 346.088 l 220.379 346.088 m 220.379 346.088 l
220.379 346.088 m 220.379 346.088 l 220.379 346.088 m 285.689
311.748 l 285.689 311.748 m 285.689 311.748 l 285.689 311.748 m
285.689 311.748 l 285.689 311.748 m 333.621 336.950 l 333.621
336.950 m 333.621 336.950 l 333.621 336.950 m 333.621 336.950 l
333.621 336.950 m 278.654 365.852 l 278.654 365.852 m 278.654
365.852 l 278.654 365.852 m 278.654 365.852 l 278.654 365.852 m
220.379 335.211 l 220.379 335.211 m 220.379 335.211 l 220.379
335.211 m 220.379 335.211 l 220.379 335.211 m 265.003 311.748 l
265.003 311.748 m 265.003 311.748 l 265.003 311.748 m 265.003
311.748 l 265.003 311.748 m 333.621 347.827 l 333.621 347.827 m
333.621 347.827 l 333.621 347.827 m 333.621 347.827 l 333.621
347.827 m 291.129 370.169 l 291.129 370.169 m 291.129 370.169 l
291.129 370.169 m 291.129 370.169 l 291.129 370.169 m 353.668
403.052 l 353.668 403.052 m 353.668 403.052 l 353.668 403.052 m
353.668 403.052 l 353.668 403.052 m 404.371 376.392 l 404.371
376.392 m 404.371 376.392 l 404.371 376.392 m 404.371 376.392 l
404.371 376.392 m 352.175 348.948 l 352.175 348.948 m 352.175
348.948 l 352.175 348.948 m 352.175 348.948 l 352.175 348.948 m
291.129 381.046 l 291.129 381.046 m 291.129 381.046 l 291.129
381.046 m 291.129 381.046 l 291.129 381.046 m 333.621 403.388 l
333.621 403.388 m 333.621 403.388 l 333.621 403.388 m 333.621
403.388 l 333.621 403.388 m 263.511 440.252 l 263.511 440.252 m
263.511 440.252 l 263.511 440.252 m 263.511 440.252 l 263.511
440.252 m 220.379 417.573 l 220.379 417.573 m 220.379 417.573 l
220.379 417.573 m 220.379 417.573 l 220.379 417.573 m 280.146
386.148 l 280.146 386.148 m 280.146 386.148 l 280.146 386.148 m
280.146 386.148 l 280.146 386.148 m 333.621 414.265 l 333.621
414.265 m 333.621 414.265 l 333.621 414.265 m 333.621 414.265 l
333.621 414.265 m 284.197 440.252 l 284.197 440.252 m 284.197
440.252 l 284.197 440.252 m 284.197 440.252 l 284.197 440.252 m
220.379 406.697 l 220.379 406.697 m 220.379 406.697 l 220.379
406.697 m 220.379 406.697 l stroke 220.379 406.697 m 262.871 384.354
l 262.871 384.354 m 262.871 384.354 l 262.871 384.354 m 262.871
384.354 l 262.871 384.354 m 195.532 348.948 l 195.532 348.948 m
195.532 348.948 l 195.532 348.948 m 195.532 348.948 l 195.532
348.948 m 149.629 373.084 l 149.629 373.084 m 149.629 373.084 l
149.629 373.084 m 149.629 373.084 l 149.629 373.084 m 206.625
403.052 l 206.625 403.052 m 206.625 403.052 l 206.625 403.052 m
206.625 403.052 l 206.625 403.052 m 262.871 373.478 l 262.871
373.478 m 262.871 373.478 l 262.871 373.478 m 262.871 373.478 l
262.871 373.478 m 216.218 348.948 l 216.218 348.948 m 216.218
348.948 l 216.218 348.948 m 216.218 348.948 l 216.218 348.948 m
149.629 383.960 l 149.629 383.960 m 149.629 383.960 l 149.629
383.960 m 149.629 383.960 l 149.629 383.960 m 192.121 406.303 l
192.121 406.303 m 192.121 406.303 l 192.121 406.303 m 192.121
406.303 l 192.121 406.303 m 127.554 440.252 l 127.554 440.252 m
127.554 440.252 l 127.554 440.252 m 127.554 440.252 l 127.554
440.252 m 78.879 414.659 l 78.879 414.659 m 78.879 414.659 l 78.879
414.659 m 78.879 414.659 l 78.879 414.659 m 133.104 386.148 l
133.104 386.148 m 133.104 386.148 l 133.104 386.148 m 133.104
386.148 l 133.104 386.148 m 192.121 417.179 l 192.121 417.179 m
192.121 417.179 l 192.121 417.179 m 192.121 417.179 l 192.121
417.179 m 148.239 440.252 l 148.239 440.252 m 148.239 440.252 l
148.239 440.252 m 148.239 440.252 l 148.239 440.252 m 78.879 403.783
l 78.879 403.783 m 78.879 403.783 l 78.879 403.783 m 78.879 403.783
l 78.879 403.783 m 121.371 381.440 l 121.371 381.440 m 121.371
381.440 l 121.371 381.440 m 121.371 381.440 l 121.371 381.440 m
59.575 348.948 l 59.575 348.948 m 59.575 348.948 l 59.575 348.948 m
59.575 348.948 l 59.575 348.948 m 8.129 375.998 l 8.129 375.998 m
8.129 375.998 l 8.129 375.998 m 8.129 375.998 l 8.129 375.998 m
59.582 403.052 l 59.582 403.052 m 59.582 403.052 l 59.582 403.052 m
59.582 403.052 l 59.582 403.052 m 121.371 370.564 l 121.371 370.564
m 121.371 370.564 l 121.371 370.564 m 121.371 370.564 l 121.371
370.564 m 78.879 348.221 l 78.879 348.221 m 78.879 348.221 l 78.879
348.221 m 78.879 348.221 l 78.879 348.221 m 148.247 311.748 l
148.247 311.748 m 148.247 311.748 l 148.247 311.748 m 148.247
311.748 l 148.247 311.748 m 192.121 334.817 l 192.121 334.817 m
192.121 334.817 l 192.121 334.817 m 192.121 334.817 l 192.121
334.817 m 133.096 365.852 l 133.096 365.852 m 133.096 365.852 l
133.096 365.852 m 133.096 365.852 l 133.096 365.852 m 78.879 337.345
l 78.879 337.345 m 78.879 337.345 l 78.879 337.345 m 78.879 337.345
l 78.879 337.345 m 127.561 311.748 l 127.561 311.748 m 127.561
311.748 l 127.561 311.748 m 127.561 311.748 l 127.561 311.748 m
192.121 345.693 l 192.121 345.693 m 192.121 345.693 l 192.121
345.693 m 192.121 345.693 l 192.121 345.693 m 149.629 368.036 l
149.629 368.036 m 149.629 368.036 l 149.629 368.036 m 149.629
368.036 l 149.629 368.036 m 216.225 403.052 l 216.225 403.052 m
216.225 403.052 l 216.225 403.052 m 216.225 403.052 l 216.225
403.052 m 262.871 378.526 l 262.871 378.526 m 262.871 378.526 l
262.871 378.526 m 262.871 378.526 l 262.871 378.526 m 206.618
348.948 l 206.618 348.948 m 206.618 348.948 l 206.618 348.948 m
206.618 348.948 l 206.618 348.948 m 149.629 378.912 l 149.629
378.912 m 149.629 378.912 l 149.629 378.912 m 149.629 378.912 l
149.629 378.912 m 195.539 403.052 l 195.539 403.052 m 195.539
403.052 l 195.539 403.052 m 195.539 403.052 l 195.539 403.052 m
262.871 367.649 l 262.871 367.649 m 262.871 367.649 l 262.871
367.649 m 262.871 367.649 l 262.871 367.649 m 220.379 345.307 l
220.379 345.307 m 220.379 345.307 l 220.379 345.307 m 220.379
345.307 l 220.379 345.307 m 284.204 311.748 l 284.204 311.748 m
284.204 311.748 l 284.204 311.748 m 284.204 311.748 l 284.204
311.748 m 333.621 337.731 l 333.621 337.731 m 333.621 337.731 l
333.621 337.731 m 333.621 337.731 l 333.621 337.731 m 280.139
365.852 l 280.139 365.852 m 280.139 365.852 l 280.139 365.852 m
280.139 365.852 l 280.139 365.852 m 220.379 334.430 l 220.379
334.430 m 220.379 334.430 l 220.379 334.430 m 220.379 334.430 l
220.379 334.430 m 263.518 311.748 l 263.518 311.748 m 263.518
311.748 l 263.518 311.748 m 263.518 311.748 l 263.518 311.748 m
333.621 348.608 l 333.621 348.608 m 333.621 348.608 l 333.621
348.608 m 333.621 348.608 l 333.621 348.608 m 291.129 370.950 l
291.129 370.950 m 291.129 370.950 l 291.129 370.950 m 291.129
370.950 l 291.129 370.950 m 352.182 403.052 l 352.182 403.052 m
352.182 403.052 l 352.182 403.052 m 352.182 403.052 l 352.182
403.052 m 404.371 375.611 l 404.371 375.611 m 404.371 375.611 l
404.371 375.611 m 404.371 375.611 l 404.371 375.611 m 353.660
348.948 l 353.660 348.948 m 353.660 348.948 l 353.660 348.948 m
353.660 348.948 l 353.660 348.948 m 291.129 381.827 l 291.129
381.827 m 291.129 381.827 l 291.129 381.827 m 291.129 381.827 l
291.129 381.827 m 333.621 404.169 l 333.621 404.169 m 333.621
404.169 l 333.621 404.169 m 333.621 404.169 l 333.621 404.169 m
264.996 440.252 l 264.996 440.252 m 264.996 440.252 l 264.996
440.252 m 264.996 440.252 l 264.996 440.252 m 220.379 416.793 l
220.379 416.793 m 220.379 416.793 l 220.379 416.793 m 220.379
416.793 l 220.379 416.793 m 278.661 386.148 l 278.661 386.148 m
278.661 386.148 l 278.661 386.148 m 278.661 386.148 l 278.661
386.148 m 333.621 415.046 l 333.621 415.046 m 333.621 415.046 l
333.621 415.046 m 333.621 415.046 l 333.621 415.046 m 285.682
440.252 l 285.682 440.252 m 285.682 440.252 l 285.682 440.252 m
285.682 440.252 l 285.682 440.252 m 220.379 405.916 l 220.379
405.916 m 220.379 405.916 l 220.379 405.916 m 220.379 405.916 l
220.379 405.916 m 262.871 383.574 l 262.871 383.574 m 262.871
383.574 l 262.871 383.574 m 262.871 383.574 l 262.871 383.574 m
197.017 348.948 l 197.017 348.948 m 197.017 348.948 l 197.017
348.948 m 197.017 348.948 l 197.017 348.948 m 149.629 373.865 l
149.629 373.865 m 149.629 373.865 l 149.629 373.865 m 149.629
373.865 l 149.629 373.865 m 205.140 403.052 l 205.140 403.052 m
205.140 403.052 l 205.140 403.052 m 205.140 403.052 l 205.140
403.052 m 262.871 372.697 l 262.871 372.697 m 262.871 372.697 l
262.871 372.697 m 262.871 372.697 l 262.871 372.697 m 217.703
348.948 l 217.703 348.948 m 217.703 348.948 l 217.703 348.948 m
217.703 348.948 l 217.703 348.948 m 149.629 384.741 l 149.629
384.741 m 149.629 384.741 l 149.629 384.741 m 149.629 384.741 l
149.629 384.741 m 192.121 407.084 l 192.121 407.084 m 192.121
407.084 l 192.121 407.084 m 192.121 407.084 l 192.121 407.084 m
129.039 440.252 l 129.039 440.252 m 129.039 440.252 l 129.039
440.252 m 129.039 440.252 l 129.039 440.252 m 78.879 413.878 l
78.879 413.878 m 78.879 413.878 l 78.879 413.878 m 78.879 413.878 l
78.879 413.878 m 131.618 386.148 l 131.618 386.148 m 131.618 386.148
l 131.618 386.148 m 131.618 386.148 l 131.618 386.148 m 192.121
417.960 l 192.121 417.960 m 192.121 417.960 l 192.121 417.960 m
192.121 417.960 l 192.121 417.960 m 149.629 440.303 l 149.629
440.303 m 149.629 440.303 l 149.629 440.303 m 149.629 440.303 l
149.629 440.303 m 220.283 477.452 l 220.283 477.452 m 220.283
477.452 l 220.283 477.452 m 220.283 477.452 l 220.283 477.452 m
262.871 455.059 l 262.871 455.059 m 262.871 455.059 l 262.871
455.059 m 262.871 455.059 l 262.871 455.059 m 202.560 423.348 l
202.560 423.348 m 202.560 423.348 l 202.560 423.348 m 202.560
423.348 l 202.560 423.348 m 149.629 451.179 l 149.629 451.179 m
149.629 451.179 l 149.629 451.179 m 149.629 451.179 l 149.629
451.179 m 199.597 477.452 l 199.597 477.452 m 199.597 477.452 l
199.597 477.452 m 199.597 477.452 l 199.597 477.452 m 262.871
444.183 l 262.871 444.183 m 262.871 444.183 l 262.871 444.183 m
262.871 444.183 l 262.871 444.183 m 220.379 421.840 l 220.379
421.840 m 220.379 421.840 l 220.379 421.840 m 220.379 421.840 l
220.379 421.840 m 288.261 386.148 l 288.261 386.148 m 288.261
386.148 l 288.261 386.148 m 288.261 386.148 l 288.261 386.148 m
333.621 409.998 l 333.621 409.998 m 333.621 409.998 l 333.621
409.998 m 333.621 409.998 l 333.621 409.998 m 276.081 440.252 l
276.081 440.252 m 276.081 440.252 l 276.081 440.252 m 276.081
440.252 l 276.081 440.252 m 220.379 410.964 l 220.379 410.964 m
220.379 410.964 l 220.379 410.964 m 220.379 410.964 l 220.379
410.964 m 267.576 386.148 l 267.576 386.148 m 267.576 386.148 l
267.576 386.148 m 267.576 386.148 l 267.576 386.148 m 333.621
420.874 l 333.621 420.874 m 333.621 420.874 l 333.621 420.874 m
333.621 420.874 l 333.621 420.874 m 291.129 443.217 l 291.129
443.217 m 291.129 443.217 l 291.129 443.217 m 291.129 443.217 l
291.129 443.217 m 356.240 477.452 l 356.240 477.452 m 356.240
477.452 l 356.240 477.452 m 356.240 477.452 l 356.240 477.452 m
404.371 452.145 l 404.371 452.145 m 404.371 452.145 l 404.371
452.145 m 404.371 452.145 l 404.371 452.145 m 349.603 423.348 l
349.603 423.348 m 349.603 423.348 l 349.603 423.348 m 349.603
423.348 l 349.603 423.348 m 291.129 454.093 l 291.129 454.093 m
291.129 454.093 l 291.129 454.093 m 291.129 454.093 l 291.129
454.093 m 335.554 477.452 l 335.554 477.452 m 335.554 477.452 l
stroke 335.554 477.452 m 335.554 477.452 l 335.554 477.452 m 404.371
441.268 l 404.371 441.268 m 404.371 441.268 l 404.371 441.268 m
404.371 441.268 l 404.371 441.268 m 361.879 418.926 l 361.879
418.926 m 361.879 418.926 l 361.879 418.926 m 361.879 418.926 l
361.879 418.926 m 424.219 386.148 l 424.219 386.148 m 424.219
386.148 l 424.219 386.148 m 424.219 386.148 l 424.219 386.148 m
475.121 412.912 l 475.121 412.912 m 475.121 412.912 l 475.121
412.912 m 475.121 412.912 l 475.121 412.912 m 423.124 440.252 l
423.124 440.252 m 423.124 440.252 l 423.124 440.252 m 423.124
440.252 l 423.124 440.252 m 361.879 408.050 l 361.879 408.050 m
361.879 408.050 l 361.879 408.050 m 361.879 408.050 l 361.879
408.050 m 404.371 385.707 l 404.371 385.707 m 404.371 385.707 l
404.371 385.707 m 404.371 385.707 l 404.371 385.707 m 334.460
348.948 l 334.460 348.948 m 334.460 348.948 l 334.460 348.948 m
334.460 348.948 l 334.460 348.948 m 291.129 371.731 l 291.129
371.731 m 291.129 371.731 l 291.129 371.731 m 291.129 371.731 l
291.129 371.731 m 350.697 403.052 l 350.697 403.052 m 350.697
403.052 l 350.697 403.052 m 350.697 403.052 l 350.697 403.052 m
404.371 374.831 l 404.371 374.831 m 404.371 374.831 l 404.371
374.831 m 404.371 374.831 l 404.371 374.831 m 355.146 348.948 l
355.146 348.948 m 355.146 348.948 l 355.146 348.948 m 355.146
348.948 l 355.146 348.948 m 291.129 382.608 l 291.129 382.608 m
291.129 382.608 l 291.129 382.608 m 291.129 382.608 l 291.129
382.608 m 333.621 404.950 l 333.621 404.950 m 333.621 404.950 l
333.621 404.950 m 333.621 404.950 l 333.621 404.950 m 266.481
440.252 l 266.481 440.252 m 266.481 440.252 l 266.481 440.252 m
266.481 440.252 l 266.481 440.252 m 220.379 416.012 l 220.379
416.012 m 220.379 416.012 l 220.379 416.012 m 220.379 416.012 l
220.379 416.012 m 277.176 386.148 l 277.176 386.148 m 277.176
386.148 l 277.176 386.148 m 277.176 386.148 l 277.176 386.148 m
333.621 415.827 l 333.621 415.827 m 333.621 415.827 l 333.621
415.827 m 333.621 415.827 l 333.621 415.827 m 287.167 440.252 l
287.167 440.252 m 287.167 440.252 l 287.167 440.252 m 287.167
440.252 l 287.167 440.252 m 220.379 405.135 l 220.379 405.135 m
220.379 405.135 l 220.379 405.135 m 220.379 405.135 l 220.379
405.135 m 262.871 382.793 l 262.871 382.793 m 262.871 382.793 l
262.871 382.793 m 262.871 382.793 l 262.871 382.793 m 198.503
348.948 l 198.503 348.948 m 198.503 348.948 l 198.503 348.948 m
198.503 348.948 l 198.503 348.948 m 149.629 374.646 l 149.629
374.646 m 149.629 374.646 l 149.629 374.646 m 149.629 374.646 l
149.629 374.646 m 203.655 403.052 l 203.655 403.052 m 203.655
403.052 l 203.655 403.052 m 203.655 403.052 l 203.655 403.052 m
262.871 371.916 l 262.871 371.916 m 262.871 371.916 l 262.871
371.916 m 262.871 371.916 l 262.871 371.916 m 219.188 348.948 l
219.188 348.948 m 219.188 348.948 l 219.188 348.948 m 219.188
348.948 l 219.188 348.948 m 149.629 385.522 l 149.629 385.522 m
149.629 385.522 l 149.629 385.522 m 149.629 385.522 l 149.629
385.522 m 192.121 407.864 l 192.121 407.864 m 192.121 407.864 l
192.121 407.864 m 192.121 407.864 l 192.121 407.864 m 130.524
440.252 l 130.524 440.252 m 130.524 440.252 l 130.524 440.252 m
130.524 440.252 l 130.524 440.252 m 78.879 413.097 l 78.879 413.097
m 78.879 413.097 l 78.879 413.097 m 78.879 413.097 l 78.879 413.097
m 130.133 386.148 l 130.133 386.148 m 130.133 386.148 l 130.133
386.148 m 130.133 386.148 l 130.133 386.148 m 192.121 418.741 l
192.121 418.741 m 192.121 418.741 l 192.121 418.741 m 192.121
418.741 l 192.121 418.741 m 149.629 441.083 l 149.629 441.083 m
149.629 441.083 l 149.629 441.083 m 149.629 441.083 l 149.629
441.083 m 218.798 477.452 l 218.798 477.452 m 218.798 477.452 l
218.798 477.452 m 218.798 477.452 l 218.798 477.452 m 262.871
454.278 l 262.871 454.278 m 262.871 454.278 l 262.871 454.278 m
262.871 454.278 l 262.871 454.278 m 204.045 423.348 l 204.045
423.348 m 204.045 423.348 l 204.045 423.348 m 204.045 423.348 l
204.045 423.348 m 149.629 451.960 l 149.629 451.960 m 149.629
451.960 l 149.629 451.960 m 149.629 451.960 l 149.629 451.960 m
198.112 477.452 l 198.112 477.452 m 198.112 477.452 l 198.112
477.452 m 198.112 477.452 l 198.112 477.452 m 262.871 443.402 l
262.871 443.402 m 262.871 443.402 l 262.871 443.402 m 262.871
443.402 l 262.871 443.402 m 220.379 421.059 l 220.379 421.059 m
220.379 421.059 l 220.379 421.059 m 220.379 421.059 l 220.379
421.059 m 286.776 386.148 l 286.776 386.148 m 286.776 386.148 l
286.776 386.148 m 286.776 386.148 l 286.776 386.148 m 333.621
410.779 l 333.621 410.779 m 333.621 410.779 l 333.621 410.779 m
333.621 410.779 l 333.621 410.779 m 277.567 440.252 l 277.567
440.252 m 277.567 440.252 l 277.567 440.252 m 277.567 440.252 l
277.567 440.252 m 220.379 410.183 l 220.379 410.183 m 220.379
410.183 l 220.379 410.183 m 220.379 410.183 l 220.379 410.183 m
266.090 386.148 l 266.090 386.148 m 266.090 386.148 l 266.090
386.148 m 266.090 386.148 l 266.090 386.148 m 333.621 421.655 l
333.621 421.655 m 333.621 421.655 l 333.621 421.655 m 333.621
421.655 l 333.621 421.655 m 291.129 443.998 l 291.129 443.998 m
291.129 443.998 l 291.129 443.998 m 291.129 443.998 l 291.129
443.998 m 354.755 477.452 l 354.755 477.452 m 354.755 477.452 l
354.755 477.452 m 354.755 477.452 l 354.755 477.452 m 404.371
451.364 l 404.371 451.364 m 404.371 451.364 l 404.371 451.364 m
404.371 451.364 l 404.371 451.364 m 351.088 423.348 l 351.088
423.348 m 351.088 423.348 l 351.088 423.348 m 351.088 423.348 l
351.088 423.348 m 291.129 454.874 l 291.129 454.874 m 291.129
454.874 l 291.129 454.874 m 291.129 454.874 l 291.129 454.874 m
334.069 477.452 l 334.069 477.452 m 334.069 477.452 l 334.069
477.452 m 334.069 477.452 l 334.069 477.452 m 404.371 440.488 l
404.371 440.488 m 404.371 440.488 l 404.371 440.488 m 404.371
440.488 l 404.371 440.488 m 361.879 418.145 l 361.879 418.145 m
361.879 418.145 l 361.879 418.145 m 361.879 418.145 l 361.879
418.145 m 422.734 386.148 l 422.734 386.148 m 422.734 386.148 l
422.734 386.148 m 422.734 386.148 l 422.734 386.148 m 475.121
413.693 l 475.121 413.693 m 475.121 413.693 l 475.121 413.693 m
475.121 413.693 l 475.121 413.693 m 424.609 440.252 l 424.609
440.252 m 424.609 440.252 l 424.609 440.252 m 424.609 440.252 l
424.609 440.252 m 361.879 407.269 l 361.879 407.269 m 361.879
407.269 l 361.879 407.269 m 361.879 407.269 l 361.879 407.269 m
404.371 384.926 l 404.371 384.926 m 404.371 384.926 l 404.371
384.926 m 404.371 384.926 l 404.371 384.926 m 335.945 348.948 l
335.945 348.948 m 335.945 348.948 l 335.945 348.948 m 335.945
348.948 l 335.945 348.948 m 291.129 372.512 l 291.129 372.512 m
291.129 372.512 l 291.129 372.512 m 291.129 372.512 l 291.129
372.512 m 349.212 403.052 l 349.212 403.052 m 349.212 403.052 l
349.212 403.052 m 349.212 403.052 l 349.212 403.052 m 404.371
374.050 l 404.371 374.050 m 404.371 374.050 l 404.371 374.050 m
404.371 374.050 l 404.371 374.050 m 356.631 348.948 l 356.631
348.948 m 356.631 348.948 l 356.631 348.948 m 356.631 348.948 l
356.631 348.948 m 291.129 383.389 l 291.129 383.389 m 291.129
383.389 l 291.129 383.389 m 291.129 383.389 l 291.129 383.389 m
333.621 405.731 l 333.621 405.731 m 333.621 405.731 l 333.621
405.731 m 333.621 405.731 l 333.621 405.731 m 267.966 440.252 l
267.966 440.252 m 267.966 440.252 l 267.966 440.252 m 267.966
440.252 l 267.966 440.252 m 220.379 415.231 l 220.379 415.231 m
220.379 415.231 l 220.379 415.231 m 220.379 415.231 l 220.379
415.231 m 275.691 386.148 l 275.691 386.148 m 275.691 386.148 l
275.691 386.148 m 275.691 386.148 l 275.691 386.148 m 333.621
416.607 l 333.621 416.607 m 333.621 416.607 l 333.621 416.607 m
333.621 416.607 l 333.621 416.607 m 288.652 440.252 l 288.652
440.252 m 288.652 440.252 l 288.652 440.252 m 288.652 440.252 l
288.652 440.252 m 220.379 404.354 l 220.379 404.354 m 220.379
404.354 l 220.379 404.354 m 220.379 404.354 l 220.379 404.354 m
262.871 382.012 l 262.871 382.012 m 262.871 382.012 l 262.871
382.012 m 262.871 382.012 l 262.871 382.012 m 199.988 348.948 l
199.988 348.948 m 199.988 348.948 l 199.988 348.948 m 199.988
348.948 l 199.988 348.948 m 149.629 375.426 l 149.629 375.426 m
149.629 375.426 l 149.629 375.426 m 149.629 375.426 l 149.629
375.426 m 202.169 403.052 l 202.169 403.052 m 202.169 403.052 l
202.169 403.052 m 202.169 403.052 l 202.169 403.052 m 262.871
371.135 l 262.871 371.135 m 262.871 371.135 l 262.871 371.135 m
262.871 371.135 l 262.871 371.135 m 220.379 348.793 l 220.379
348.793 m 220.379 348.793 l 220.379 348.793 m 220.379 348.793 l
220.379 348.793 m 290.834 311.748 l 290.834 311.748 m 290.834
311.748 l 290.834 311.748 m 290.834 311.748 l 290.834 311.748 m
333.621 334.245 l 333.621 334.245 m 333.621 334.245 l 333.621
334.245 m 333.621 334.245 l 333.621 334.245 m 273.509 365.852 l
273.509 365.852 m 273.509 365.852 l 273.509 365.852 m 273.509
365.852 l 273.509 365.852 m 220.379 337.916 l 220.379 337.916 m
220.379 337.916 l 220.379 337.916 m 220.379 337.916 l 220.379
337.916 m 270.148 311.748 l 270.148 311.748 m 270.148 311.748 l
270.148 311.748 m 270.148 311.748 l 270.148 311.748 m 333.621
345.122 l stroke 333.621 345.122 m 333.621 345.122 l 333.621 345.122
m 333.621 345.122 l 333.621 345.122 m 291.129 367.464 l 291.129
367.464 m 291.129 367.464 l 291.129 367.464 m 291.129 367.464 l
291.129 367.464 m 358.812 403.052 l 358.812 403.052 m 358.812
403.052 l 358.812 403.052 m 358.812 403.052 l 358.812 403.052 m
404.371 379.097 l 404.371 379.097 m 404.371 379.097 l 404.371
379.097 m 404.371 379.097 l 404.371 379.097 m 347.030 348.948 l
347.030 348.948 m 347.030 348.948 l 347.030 348.948 m 347.030
348.948 l 347.030 348.948 m 291.129 378.341 l 291.129 378.341 m
291.129 378.341 l 291.129 378.341 m 291.129 378.341 l 291.129
378.341 m 338.127 403.052 l 338.127 403.052 m 338.127 403.052 l
338.127 403.052 m 338.127 403.052 l 338.127 403.052 m 404.371
368.221 l 404.371 368.221 m 404.371 368.221 l 404.371 368.221 m
404.371 368.221 l 404.371 368.221 m 361.879 345.879 l 361.879
345.879 m 361.879 345.879 l 361.879 345.879 m 361.879 345.879 l
361.879 345.879 m 426.791 311.748 l 426.791 311.748 m 426.791
311.748 l 426.791 311.748 m 426.791 311.748 l 426.791 311.748 m
475.121 337.160 l 475.121 337.160 m 475.121 337.160 l 475.121
337.160 m 475.121 337.160 l 475.121 337.160 m 420.552 365.852 l
420.552 365.852 m 420.552 365.852 l 420.552 365.852 m 420.552
365.852 l 420.552 365.852 m 361.879 335.002 l 361.879 335.002 m
361.879 335.002 l 361.879 335.002 m 361.879 335.002 l 361.879
335.002 m 406.105 311.748 l 406.105 311.748 m 406.105 311.748 l
406.105 311.748 m 406.105 311.748 l 406.105 311.748 m 475.121
348.036 l 475.121 348.036 m 475.121 348.036 l 475.121 348.036 m
475.121 348.036 l 475.121 348.036 m 432.629 370.379 l 432.629
370.379 m 432.629 370.379 l 432.629 370.379 m 432.629 370.379 l
432.629 370.379 m 494.770 403.052 l 494.770 403.052 m 494.770
403.052 l 494.770 403.052 m 494.770 403.052 l 494.770 403.052 m
545.871 376.183 l 545.871 376.183 m 545.871 376.183 l 545.871
376.183 m 545.871 376.183 l 545.871 376.183 m 494.073 348.948 l
494.073 348.948 m 494.073 348.948 l 494.073 348.948 m 494.073
348.948 l 494.073 348.948 m 432.629 381.255 l 432.629 381.255 m
432.629 381.255 l 432.629 381.255 m 432.629 381.255 l 432.629
381.255 m 475.121 403.598 l 475.121 403.598 m 475.121 403.598 l
475.121 403.598 m 475.121 403.598 l 475.121 403.598 m 405.409
440.252 l 405.409 440.252 m 405.409 440.252 l 405.409 440.252 m
405.409 440.252 l 405.409 440.252 m 361.879 417.364 l 361.879
417.364 m 361.879 417.364 l 361.879 417.364 m 361.879 417.364 l
361.879 417.364 m 421.248 386.148 l 421.248 386.148 m 421.248
386.148 l 421.248 386.148 m 421.248 386.148 l 421.248 386.148 m
475.121 414.474 l 475.121 414.474 m 475.121 414.474 l 475.121
414.474 m 475.121 414.474 l 475.121 414.474 m 426.095 440.252 l
426.095 440.252 m 426.095 440.252 l 426.095 440.252 m 426.095
440.252 l 426.095 440.252 m 361.879 406.488 l 361.879 406.488 m
361.879 406.488 l 361.879 406.488 m 361.879 406.488 l 361.879
406.488 m 404.371 384.145 l 404.371 384.145 m 404.371 384.145 l
404.371 384.145 m 404.371 384.145 l 404.371 384.145 m 337.430
348.948 l 337.430 348.948 m 337.430 348.948 l 337.430 348.948 m
337.430 348.948 l 337.430 348.948 m 291.129 373.293 l 291.129
373.293 m 291.129 373.293 l 291.129 373.293 m 291.129 373.293 l
291.129 373.293 m 347.727 403.052 l 347.727 403.052 m 347.727
403.052 l 347.727 403.052 m 347.727 403.052 l 347.727 403.052 m
404.371 373.269 l 404.371 373.269 m 404.371 373.269 l 404.371
373.269 m 404.371 373.269 l 404.371 373.269 m 358.116 348.948 l
358.116 348.948 m 358.116 348.948 l 358.116 348.948 m 358.116
348.948 l 358.116 348.948 m 291.129 384.169 l 291.129 384.169 m
291.129 384.169 l 291.129 384.169 m 291.129 384.169 l 291.129
384.169 m 333.621 406.512 l 333.621 406.512 m 333.621 406.512 l
333.621 406.512 m 333.621 406.512 l 333.621 406.512 m 269.452
440.252 l 269.452 440.252 m 269.452 440.252 l 269.452 440.252 m
269.452 440.252 l 269.452 440.252 m 220.379 414.450 l 220.379
414.450 m 220.379 414.450 l 220.379 414.450 m 220.379 414.450 l
220.379 414.450 m 274.206 386.148 l 274.206 386.148 m 274.206
386.148 l 274.206 386.148 m 274.206 386.148 l 274.206 386.148 m
333.621 417.388 l 333.621 417.388 m 333.621 417.388 l 333.621
417.388 m 333.621 417.388 l 333.621 417.388 m 290.137 440.252 l
290.137 440.252 m 290.137 440.252 l 290.137 440.252 m 290.137
440.252 l 290.137 440.252 m 220.379 403.573 l 220.379 403.573 m
220.379 403.573 l 220.379 403.573 m 220.379 403.573 l 220.379
403.573 m 262.871 381.231 l 262.871 381.231 m 262.871 381.231 l
262.871 381.231 m 262.871 381.231 l 262.871 381.231 m 201.473
348.948 l 201.473 348.948 m 201.473 348.948 l 201.473 348.948 m
201.473 348.948 l 201.473 348.948 m 149.629 376.207 l 149.629
376.207 m 149.629 376.207 l 149.629 376.207 m 149.629 376.207 l
149.629 376.207 m 200.684 403.052 l 200.684 403.052 m 200.684
403.052 l 200.684 403.052 m 200.684 403.052 l 200.684 403.052 m
262.871 370.354 l 262.871 370.354 m 262.871 370.354 l 262.871
370.354 m 262.871 370.354 l 262.871 370.354 m 220.379 348.012 l
220.379 348.012 m 220.379 348.012 l 220.379 348.012 m 220.379
348.012 l 220.379 348.012 m 289.349 311.748 l 289.349 311.748 m
289.349 311.748 l 289.349 311.748 m 289.349 311.748 l 289.349
311.748 m 333.621 335.026 l 333.621 335.026 m 333.621 335.026 l
333.621 335.026 m 333.621 335.026 l 333.621 335.026 m 274.994
365.852 l 274.994 365.852 m 274.994 365.852 l 274.994 365.852 m
274.994 365.852 l 274.994 365.852 m 220.379 337.135 l 220.379
337.135 m 220.379 337.135 l 220.379 337.135 m 220.379 337.135 l
220.379 337.135 m 268.663 311.748 l 268.663 311.748 m 268.663
311.748 l 268.663 311.748 m 268.663 311.748 l 268.663 311.748 m
333.621 345.903 l 333.621 345.903 m 333.621 345.903 l 333.621
345.903 m 333.621 345.903 l 333.621 345.903 m 291.129 368.245 l
291.129 368.245 m 291.129 368.245 l 291.129 368.245 m 291.129
368.245 l 291.129 368.245 m 357.327 403.052 l 357.327 403.052 m
357.327 403.052 l 357.327 403.052 m 357.327 403.052 l 357.327
403.052 m 404.371 378.317 l 404.371 378.317 m 404.371 378.317 l
404.371 378.317 m 404.371 378.317 l 404.371 378.317 m 348.516
348.948 l 348.516 348.948 m 348.516 348.948 l 348.516 348.948 m
348.516 348.948 l 348.516 348.948 m 291.129 379.122 l 291.129
379.122 m 291.129 379.122 l 291.129 379.122 m 291.129 379.122 l
291.129 379.122 m 336.642 403.052 l 336.642 403.052 m 336.642
403.052 l 336.642 403.052 m 336.642 403.052 l 336.642 403.052 m
404.371 367.440 l 404.371 367.440 m 404.371 367.440 l 404.371
367.440 m 404.371 367.440 l 404.371 367.440 m 361.879 345.098 l
361.879 345.098 m 361.879 345.098 l 361.879 345.098 m 361.879
345.098 l 361.879 345.098 m 425.306 311.748 l 425.306 311.748 m
425.306 311.748 l 425.306 311.748 m 425.306 311.748 l 425.306
311.748 m 475.121 337.941 l 475.121 337.941 m 475.121 337.941 l
475.121 337.941 m 475.121 337.941 l 475.121 337.941 m 422.037
365.852 l 422.037 365.852 m 422.037 365.852 l 422.037 365.852 m
422.037 365.852 l 422.037 365.852 m 361.879 334.221 l 361.879
334.221 m 361.879 334.221 l 361.879 334.221 m 361.879 334.221 l
361.879 334.221 m 404.620 311.748 l 404.620 311.748 m 404.620
311.748 l 404.620 311.748 m 404.620 311.748 l 404.620 311.748 m
475.121 348.817 l 475.121 348.817 m 475.121 348.817 l 475.121
348.817 m 475.121 348.817 l 475.121 348.817 m 432.629 371.160 l
432.629 371.160 m 432.629 371.160 l 432.629 371.160 m 432.629
371.160 l 432.629 371.160 m 493.285 403.052 l 493.285 403.052 m
493.285 403.052 l 493.285 403.052 m 493.285 403.052 l 493.285
403.052 m 545.871 375.402 l 545.871 375.402 m 545.871 375.402 l
545.871 375.402 m 545.871 375.402 l 545.871 375.402 m 495.558
348.948 l 495.558 348.948 m 495.558 348.948 l 495.558 348.948 m
495.558 348.948 l 495.558 348.948 m 432.629 382.036 l 432.629
382.036 m 432.629 382.036 l 432.629 382.036 m 432.629 382.036 l
432.629 382.036 m 475.121 404.378 l 475.121 404.378 m 475.121
404.378 l 475.121 404.378 m 475.121 404.378 l 475.121 404.378 m
406.894 440.252 l 406.894 440.252 m 406.894 440.252 l 406.894
440.252 m 406.894 440.252 l 406.894 440.252 m 361.879 416.583 l
361.879 416.583 m 361.879 416.583 l 361.879 416.583 m 361.879
416.583 l 361.879 416.583 m 419.763 386.148 l 419.763 386.148 m
419.763 386.148 l 419.763 386.148 m 419.763 386.148 l 419.763
386.148 m 475.121 415.255 l 475.121 415.255 m 475.121 415.255 l
475.121 415.255 m 475.121 415.255 l 475.121 415.255 m 427.580
440.252 l 427.580 440.252 m 427.580 440.252 l 427.580 440.252 m
427.580 440.252 l 427.580 440.252 m 361.879 405.707 l 361.879
405.707 m 361.879 405.707 l 361.879 405.707 m 361.879 405.707 l
361.879 405.707 m 404.371 383.364 l 404.371 383.364 m 404.371
383.364 l 404.371 383.364 m 404.371 383.364 l 404.371 383.364 m
338.915 348.948 l 338.915 348.948 m 338.915 348.948 l 338.915
348.948 m 338.915 348.948 l 338.915 348.948 m 291.129 374.074 l
291.129 374.074 m 291.129 374.074 l 291.129 374.074 m 291.129
374.074 l 291.129 374.074 m 346.242 403.052 l 346.242 403.052 m
346.242 403.052 l 346.242 403.052 m 346.242 403.052 l 346.242
403.052 m 404.371 372.488 l 404.371 372.488 m 404.371 372.488 l
404.371 372.488 m 404.371 372.488 l stroke 404.371 372.488 m 359.601
348.948 l 359.601 348.948 m 359.601 348.948 l 359.601 348.948 m
359.601 348.948 l 359.601 348.948 m 291.129 384.950 l 291.129
384.950 m 291.129 384.950 l 291.129 384.950 m 291.129 384.950 l
291.129 384.950 m 333.621 407.293 l 333.621 407.293 m 333.621
407.293 l 333.621 407.293 m 333.621 407.293 l 333.621 407.293 m
270.937 440.252 l 270.937 440.252 m 270.937 440.252 l 270.937
440.252 m 270.937 440.252 l 270.937 440.252 m 220.379 413.669 l
220.379 413.669 m 220.379 413.669 l 220.379 413.669 m 220.379
413.669 l 220.379 413.669 m 272.720 386.148 l 272.720 386.148 m
272.720 386.148 l 272.720 386.148 m 272.720 386.148 l 272.720
386.148 m 333.621 418.169 l 333.621 418.169 m 333.621 418.169 l
333.621 418.169 m 333.621 418.169 l 333.621 418.169 m 291.129
440.512 l 291.129 440.512 m 291.129 440.512 l 291.129 440.512 m
291.129 440.512 l 291.129 440.512 m 361.385 477.452 l 361.385
477.452 m 361.385 477.452 l 361.385 477.452 m 361.385 477.452 l
361.385 477.452 m 404.371 454.850 l 404.371 454.850 m 404.371
454.850 l 404.371 454.850 m 404.371 454.850 l 404.371 454.850 m
344.458 423.348 l 344.458 423.348 m 344.458 423.348 l 344.458
423.348 m 344.458 423.348 l 344.458 423.348 m 291.129 451.388 l
291.129 451.388 m 291.129 451.388 l 291.129 451.388 m 291.129
451.388 l 291.129 451.388 m 340.699 477.452 l 340.699 477.452 m
340.699 477.452 l 340.699 477.452 m 340.699 477.452 l 340.699
477.452 m 404.371 443.974 l 404.371 443.974 m 404.371 443.974 l
404.371 443.974 m 404.371 443.974 l 404.371 443.974 m 361.879
421.631 l 361.879 421.631 m 361.879 421.631 l 361.879 421.631 m
361.879 421.631 l 361.879 421.631 m 429.363 386.148 l 429.363
386.148 m 429.363 386.148 l 429.363 386.148 m 429.363 386.148 l
429.363 386.148 m 475.121 410.207 l 475.121 410.207 m 475.121
410.207 l 475.121 410.207 m 475.121 410.207 l 475.121 410.207 m
417.979 440.252 l 417.979 440.252 m 417.979 440.252 l 417.979
440.252 m 417.979 440.252 l 417.979 440.252 m 361.879 410.755 l
361.879 410.755 m 361.879 410.755 l 361.879 410.755 m 361.879
410.755 l 361.879 410.755 m 408.678 386.148 l 408.678 386.148 m
408.678 386.148 l 408.678 386.148 m 408.678 386.148 l 408.678
386.148 m 475.121 421.084 l 475.121 421.084 m 475.121 421.084 l
475.121 421.084 m 475.121 421.084 l 475.121 421.084 m 432.629
443.426 l 432.629 443.426 m 432.629 443.426 l 432.629 443.426 m
432.629 443.426 l 432.629 443.426 m 497.342 477.452 l 497.342
477.452 m 497.342 477.452 l 497.342 477.452 m 497.342 477.452 l
497.342 477.452 m 545.871 451.936 l 545.871 451.936 m 545.871
451.936 l 545.871 451.936 m 545.871 451.936 l 545.871 451.936 m
491.501 423.348 l 491.501 423.348 m 491.501 423.348 l 491.501
423.348 m 491.501 423.348 l 491.501 423.348 m 432.629 454.303 l
432.629 454.303 m 432.629 454.303 l 432.629 454.303 m 432.629
454.303 l 432.629 454.303 m 476.656 477.452 l 476.656 477.452 m
476.656 477.452 l 476.656 477.452 m 476.656 477.452 l 476.656
477.452 m 545.871 441.059 l 545.871 441.059 m 545.871 441.059 l
545.871 441.059 m 545.871 441.059 l 545.871 441.059 m 503.379
418.717 l 503.379 418.717 m 503.379 418.717 l 503.379 418.717 m
503.379 418.717 l 503.379 418.717 m 565.321 386.148 l 565.321
386.148 m 565.321 386.148 l 565.321 386.148 m 565.321 386.148 l
565.321 386.148 m 616.621 413.122 l 616.621 413.122 m 616.621
413.122 l 616.621 413.122 m 616.621 413.122 l 616.621 413.122 m
565.022 440.252 l 565.022 440.252 m 565.022 440.252 l 565.022
440.252 m 565.022 440.252 l 565.022 440.252 m 503.379 407.840 l
503.379 407.840 m 503.379 407.840 l 503.379 407.840 m 503.379
407.840 l 503.379 407.840 m 545.871 385.498 l 545.871 385.498 m
545.871 385.498 l 545.871 385.498 m 545.871 385.498 l 545.871
385.498 m 476.358 348.948 l 476.358 348.948 m 476.358 348.948 l
476.358 348.948 m 476.358 348.948 l 476.358 348.948 m 432.629
371.940 l 432.629 371.940 m 432.629 371.940 l 432.629 371.940 m
432.629 371.940 l 432.629 371.940 m 491.799 403.052 l 491.799
403.052 m 491.799 403.052 l 491.799 403.052 m 491.799 403.052 l
491.799 403.052 m 545.871 374.621 l 545.871 374.621 m 545.871
374.621 l 545.871 374.621 m 545.871 374.621 l 545.871 374.621 m
497.044 348.948 l 497.044 348.948 m 497.044 348.948 l 497.044
348.948 m 497.044 348.948 l 497.044 348.948 m 432.629 382.817 l
432.629 382.817 m 432.629 382.817 l 432.629 382.817 m 432.629
382.817 l 432.629 382.817 m 475.121 405.159 l 475.121 405.159 m
475.121 405.159 l 475.121 405.159 m 475.121 405.159 l 475.121
405.159 m 408.379 440.252 l 408.379 440.252 m 408.379 440.252 l
408.379 440.252 m 408.379 440.252 l 408.379 440.252 m 361.879
415.802 l 361.879 415.802 m 361.879 415.802 l 361.879 415.802 m
361.879 415.802 l 361.879 415.802 m 418.278 386.148 l 418.278
386.148 m 418.278 386.148 l 418.278 386.148 m 418.278 386.148 l
418.278 386.148 m 475.121 416.036 l 475.121 416.036 m 475.121
416.036 l 475.121 416.036 m 475.121 416.036 l 475.121 416.036 m
429.065 440.252 l 429.065 440.252 m 429.065 440.252 l 429.065
440.252 m 429.065 440.252 l 429.065 440.252 m 361.879 404.926 l
361.879 404.926 m 361.879 404.926 l 361.879 404.926 m 361.879
404.926 l 361.879 404.926 m 404.371 382.583 l 404.371 382.583 m
404.371 382.583 l 404.371 382.583 m 404.371 382.583 l 404.371
382.583 m 340.401 348.948 l 340.401 348.948 m 340.401 348.948 l
340.401 348.948 m 340.401 348.948 l 340.401 348.948 m 291.129
374.855 l 291.129 374.855 m 291.129 374.855 l 291.129 374.855 m
291.129 374.855 l 291.129 374.855 m 344.757 403.052 l 344.757
403.052 m 344.757 403.052 l 344.757 403.052 m 344.757 403.052 l
344.757 403.052 m 404.371 371.707 l 404.371 371.707 m 404.371
371.707 l 404.371 371.707 m 404.371 371.707 l 404.371 371.707 m
361.086 348.948 l 361.086 348.948 m 361.086 348.948 l 361.086
348.948 m 361.086 348.948 l 361.086 348.948 m 291.129 385.731 l
291.129 385.731 m 291.129 385.731 l 291.129 385.731 m 291.129
385.731 l 291.129 385.731 m 333.621 408.074 l 333.621 408.074 m
333.621 408.074 l 333.621 408.074 m 333.621 408.074 l 333.621
408.074 m 272.422 440.252 l 272.422 440.252 m 272.422 440.252 l
272.422 440.252 m 272.422 440.252 l 272.422 440.252 m 220.379
412.888 l 220.379 412.888 m 220.379 412.888 l 220.379 412.888 m
220.379 412.888 l 220.379 412.888 m 271.235 386.148 l 271.235
386.148 m 271.235 386.148 l 271.235 386.148 m 271.235 386.148 l
271.235 386.148 m 333.621 418.950 l 333.621 418.950 m 333.621
418.950 l 333.621 418.950 m 333.621 418.950 l 333.621 418.950 m
291.129 441.293 l 291.129 441.293 m 291.129 441.293 l 291.129
441.293 m 291.129 441.293 l 291.129 441.293 m 359.900 477.452 l
359.900 477.452 m 359.900 477.452 l 359.900 477.452 m 359.900
477.452 l 359.900 477.452 m 404.371 454.069 l 404.371 454.069 m
404.371 454.069 l 404.371 454.069 m 404.371 454.069 l 404.371
454.069 m 345.943 423.348 l 345.943 423.348 m 345.943 423.348 l
345.943 423.348 m 345.943 423.348 l 345.943 423.348 m 291.129
452.169 l 291.129 452.169 m 291.129 452.169 l 291.129 452.169 m
291.129 452.169 l 291.129 452.169 m 339.214 477.452 l 339.214
477.452 m 339.214 477.452 l 339.214 477.452 m 339.214 477.452 l
339.214 477.452 m 404.371 443.193 l 404.371 443.193 m 404.371
443.193 l 404.371 443.193 m 404.371 443.193 l 404.371 443.193 m
361.879 420.850 l 361.879 420.850 m 361.879 420.850 l 361.879
420.850 m 361.879 420.850 l 361.879 420.850 m 427.878 386.148 l
427.878 386.148 m 427.878 386.148 l 427.878 386.148 m 427.878
386.148 l 427.878 386.148 m 475.121 410.988 l 475.121 410.988 m
475.121 410.988 l 475.121 410.988 m 475.121 410.988 l 475.121
410.988 m 419.465 440.252 l 419.465 440.252 m 419.465 440.252 l
419.465 440.252 m 419.465 440.252 l 419.465 440.252 m 361.879
409.974 l 361.879 409.974 m 361.879 409.974 l 361.879 409.974 m
361.879 409.974 l 361.879 409.974 m 407.193 386.148 l 407.193
386.148 m 407.193 386.148 l 407.193 386.148 m 407.193 386.148 l
407.193 386.148 m 475.121 421.865 l 475.121 421.865 m 475.121
421.865 l 475.121 421.865 m 475.121 421.865 l 475.121 421.865 m
432.629 444.207 l 432.629 444.207 m 432.629 444.207 l 432.629
444.207 m 432.629 444.207 l 432.629 444.207 m 495.857 477.452 l
495.857 477.452 m 495.857 477.452 l 495.857 477.452 m 495.857
477.452 l 495.857 477.452 m 545.871 451.155 l 545.871 451.155 m
545.871 451.155 l 545.871 451.155 m 545.871 451.155 l 545.871
451.155 m 492.986 423.348 l 492.986 423.348 m 492.986 423.348 l
492.986 423.348 m 492.986 423.348 l 492.986 423.348 m 432.629
455.083 l 432.629 455.083 m 432.629 455.083 l 432.629 455.083 m
432.629 455.083 l 432.629 455.083 m 475.171 477.452 l 475.171
477.452 m 475.171 477.452 l 475.171 477.452 m 475.171 477.452 l
475.171 477.452 m 545.871 440.278 l 545.871 440.278 m 545.871
440.278 l 545.871 440.278 m 545.871 440.278 l 545.871 440.278 m
503.379 417.936 l 503.379 417.936 m 503.379 417.936 l 503.379
417.936 m 503.379 417.936 l 503.379 417.936 m 563.836 386.148 l
563.836 386.148 m 563.836 386.148 l 563.836 386.148 m 563.836
386.148 l 563.836 386.148 m 616.621 413.902 l 616.621 413.902 m
616.621 413.902 l 616.621 413.902 m 616.621 413.902 l 616.621
413.902 m 566.507 440.252 l 566.507 440.252 m 566.507 440.252 l
stroke 566.507 440.252 m 566.507 440.252 l 566.507 440.252 m 503.379
407.059 l 503.379 407.059 m 503.379 407.059 l 503.379 407.059 m
503.379 407.059 l 503.379 407.059 m 545.871 384.717 l 545.871
384.717 m 545.871 384.717 l 545.871 384.717 m 545.871 384.717 l
545.871 384.717 m 477.843 348.948 l 477.843 348.948 m 477.843
348.948 l 477.843 348.948 m 477.843 348.948 l 477.843 348.948 m
432.629 372.721 l 432.629 372.721 m 432.629 372.721 l 432.629
372.721 m 432.629 372.721 l 432.629 372.721 m 490.314 403.052 l
490.314 403.052 m 490.314 403.052 l 490.314 403.052 m 490.314
403.052 l 490.314 403.052 m 545.871 373.840 l 545.871 373.840 m
545.871 373.840 l 545.871 373.840 m 545.871 373.840 l 545.871
373.840 m 498.529 348.948 l 498.529 348.948 m 498.529 348.948 l
498.529 348.948 m 498.529 348.948 l 498.529 348.948 m 432.629
383.598 l 432.629 383.598 m 432.629 383.598 l 432.629 383.598 m
432.629 383.598 l 432.629 383.598 m 475.121 405.940 l 475.121
405.940 m 475.121 405.940 l 475.121 405.940 m 475.121 405.940 l
475.121 405.940 m 409.864 440.252 l 409.864 440.252 m 409.864
440.252 l 409.864 440.252 m 409.864 440.252 l 409.864 440.252 m
361.879 415.021 l 361.879 415.021 m 361.879 415.021 l 361.879
415.021 m 361.879 415.021 l 361.879 415.021 m 416.793 386.148 l
416.793 386.148 m 416.793 386.148 l 416.793 386.148 m 416.793
386.148 l 416.793 386.148 m 475.121 416.817 l 475.121 416.817 m
475.121 416.817 l 475.121 416.817 m 475.121 416.817 l 475.121
416.817 m 430.550 440.252 l 430.550 440.252 m 430.550 440.252 l
430.550 440.252 m 430.550 440.252 l 430.550 440.252 m 361.879
404.145 l 361.879 404.145 m 361.879 404.145 l 361.879 404.145 m
361.879 404.145 l 361.879 404.145 m 404.371 381.803 l 404.371
381.803 m 404.371 381.803 l 404.371 381.803 m 404.371 381.803 l
404.371 381.803 m 341.886 348.948 l 341.886 348.948 m 341.886
348.948 l 341.886 348.948 m 341.886 348.948 l 341.886 348.948 m
291.129 375.636 l 291.129 375.636 m 291.129 375.636 l 291.129
375.636 m 291.129 375.636 l 291.129 375.636 m 343.271 403.052 l
343.271 403.052 m 343.271 403.052 l 343.271 403.052 m 343.271
403.052 l 343.271 403.052 m 404.371 370.926 l 404.371 370.926 m
404.371 370.926 l 404.371 370.926 m 404.371 370.926 l 404.371
370.926 m 361.879 348.584 l 361.879 348.584 m 361.879 348.584 l
361.879 348.584 m 361.879 348.584 l 361.879 348.584 m 431.936
311.748 l 431.936 311.748 m 431.936 311.748 l 431.936 311.748 m
431.936 311.748 l 431.936 311.748 m 475.121 334.455 l 475.121
334.455 m 475.121 334.455 l 475.121 334.455 m 475.121 334.455 l
475.121 334.455 m 415.407 365.852 l 415.407 365.852 m 415.407
365.852 l 415.407 365.852 m 415.407 365.852 l 415.407 365.852 m
361.879 337.707 l 361.879 337.707 m 361.879 337.707 l 361.879
337.707 m 361.879 337.707 l 361.879 337.707 m 411.250 311.748 l
411.250 311.748 m 411.250 311.748 l 411.250 311.748 m 411.250
311.748 l 411.250 311.748 m 475.121 345.331 l 475.121 345.331 m
475.121 345.331 l 475.121 345.331 m 475.121 345.331 l 475.121
345.331 m 432.629 367.674 l 432.629 367.674 m 432.629 367.674 l
432.629 367.674 m 432.629 367.674 l 432.629 367.674 m 499.914
403.052 l 499.914 403.052 m 499.914 403.052 l 499.914 403.052 m
499.914 403.052 l 499.914 403.052 m 545.871 378.888 l 545.871
378.888 m 545.871 378.888 l 545.871 378.888 m 545.871 378.888 l
545.871 378.888 m 488.928 348.948 l 488.928 348.948 m 488.928
348.948 l 488.928 348.948 m 488.928 348.948 l 488.928 348.948 m
432.629 378.550 l 432.629 378.550 m 432.629 378.550 l 432.629
378.550 m 432.629 378.550 l 432.629 378.550 m 479.229 403.052 l
479.229 403.052 m 479.229 403.052 l 479.229 403.052 m 479.229
403.052 l 479.229 403.052 m 545.871 368.012 l 545.871 368.012 m
545.871 368.012 l 545.871 368.012 m 545.871 368.012 l 545.871
368.012 m 503.379 345.669 l 503.379 345.669 m 503.379 345.669 l
503.379 345.669 m 503.379 345.669 l 503.379 345.669 m 567.893
311.748 l 567.893 311.748 m 567.893 311.748 l 567.893 311.748 m
567.893 311.748 l 567.893 311.748 m 616.621 337.369 l 616.621
337.369 m 616.621 337.369 l 616.621 337.369 m 616.621 337.369 l
616.621 337.369 m 562.450 365.852 l 562.450 365.852 m 562.450
365.852 l 562.450 365.852 m 562.450 365.852 l 562.450 365.852 m
503.379 334.793 l 503.379 334.793 m 503.379 334.793 l 503.379
334.793 m 503.379 334.793 l 503.379 334.793 m 547.207 311.748 l
547.207 311.748 m 547.207 311.748 l 547.207 311.748 m 547.207
311.748 l 547.207 311.748 m 616.621 348.245 l 616.621 348.245 m
616.621 348.245 l 616.621 348.245 m 616.621 348.245 l 616.621
348.245 m 574.129 370.588 l 574.129 370.588 m 574.129 370.588 l
574.129 370.588 m 574.129 370.588 l 574.129 370.588 m 635.872
403.052 l 635.872 403.052 m 635.872 403.052 l 635.872 403.052 m
635.872 403.052 l 635.872 403.052 m 687.371 375.974 l 687.371
375.974 m 687.371 375.974 l 687.371 375.974 m 687.371 375.974 l
687.371 375.974 m 635.971 348.948 l 635.971 348.948 m 635.971
348.948 l 635.971 348.948 m 635.971 348.948 l 635.971 348.948 m
574.129 381.464 l 574.129 381.464 m 574.129 381.464 l 574.129
381.464 m 574.129 381.464 l 574.129 381.464 m 616.621 403.807 l
616.621 403.807 m 616.621 403.807 l 616.621 403.807 m 616.621
403.807 l 616.621 403.807 m 547.307 440.252 l 547.307 440.252 m
547.307 440.252 l 547.307 440.252 m 547.307 440.252 l 547.307
440.252 m 503.379 417.155 l 503.379 417.155 m 503.379 417.155 l
503.379 417.155 m 503.379 417.155 l 503.379 417.155 m 562.350
386.148 l 562.350 386.148 m 562.350 386.148 l 562.350 386.148 m
562.350 386.148 l 562.350 386.148 m 616.621 414.683 l 616.621
414.683 m 616.621 414.683 l 616.621 414.683 m 616.621 414.683 l
616.621 414.683 m 567.992 440.252 l 567.992 440.252 m 567.992
440.252 l 567.992 440.252 m 567.992 440.252 l 567.992 440.252 m
503.379 406.278 l 503.379 406.278 m 503.379 406.278 l 503.379
406.278 m 503.379 406.278 l 503.379 406.278 m 545.871 383.936 l
545.871 383.936 m 545.871 383.936 l 545.871 383.936 m 545.871
383.936 l 545.871 383.936 m 479.328 348.948 l 479.328 348.948 m
479.328 348.948 l 479.328 348.948 m 479.328 348.948 l 479.328
348.948 m 432.629 373.502 l 432.629 373.502 m 432.629 373.502 l
432.629 373.502 m 432.629 373.502 l 432.629 373.502 m 488.829
403.052 l 488.829 403.052 m 488.829 403.052 l 488.829 403.052 m
488.829 403.052 l 488.829 403.052 m 545.871 373.060 l 545.871
373.060 m 545.871 373.060 l 545.871 373.060 m 545.871 373.060 l
545.871 373.060 m 500.014 348.948 l 500.014 348.948 m 500.014
348.948 l 500.014 348.948 m 500.014 348.948 l 500.014 348.948 m
432.629 384.379 l 432.629 384.379 m 432.629 384.379 l 432.629
384.379 m 432.629 384.379 l 432.629 384.379 m 475.121 406.721 l
475.121 406.721 m 475.121 406.721 l 475.121 406.721 m 475.121
406.721 l 475.121 406.721 m 411.349 440.252 l 411.349 440.252 m
411.349 440.252 l 411.349 440.252 m 411.349 440.252 l 411.349
440.252 m 361.879 414.241 l 361.879 414.241 m 361.879 414.241 l
361.879 414.241 m 361.879 414.241 l 361.879 414.241 m 415.308
386.148 l 415.308 386.148 m 415.308 386.148 l 415.308 386.148 m
415.308 386.148 l 415.308 386.148 m 475.121 417.598 l 475.121
417.598 m 475.121 417.598 l 475.121 417.598 m 475.121 417.598 l
475.121 417.598 m 432.035 440.252 l 432.035 440.252 m 432.035
440.252 l 432.035 440.252 m 432.035 440.252 l 432.035 440.252 m
361.879 403.364 l 361.879 403.364 m 361.879 403.364 l 361.879
403.364 m 361.879 403.364 l 361.879 403.364 m 404.371 381.022 l
404.371 381.022 m 404.371 381.022 l 404.371 381.022 m 404.371
381.022 l 404.371 381.022 m 343.371 348.948 l 343.371 348.948 m
343.371 348.948 l 343.371 348.948 m 343.371 348.948 l 343.371
348.948 m 291.129 376.417 l 291.129 376.417 m 291.129 376.417 l
291.129 376.417 m 291.129 376.417 l 291.129 376.417 m 341.786
403.052 l 341.786 403.052 m 341.786 403.052 l 341.786 403.052 m
341.786 403.052 l 341.786 403.052 m 404.371 370.145 l 404.371
370.145 m 404.371 370.145 l 404.371 370.145 m 404.371 370.145 l
404.371 370.145 m 361.879 347.803 l 361.879 347.803 m 361.879
347.803 l 361.879 347.803 m 361.879 347.803 l 361.879 347.803 m
430.451 311.748 l 430.451 311.748 m 430.451 311.748 l 430.451
311.748 m 430.451 311.748 l 430.451 311.748 m 475.121 335.236 l
475.121 335.236 m 475.121 335.236 l 475.121 335.236 m 475.121
335.236 l 475.121 335.236 m 416.892 365.852 l 416.892 365.852 m
416.892 365.852 l 416.892 365.852 m 416.892 365.852 l 416.892
365.852 m 361.879 336.926 l 361.879 336.926 m 361.879 336.926 l
361.879 336.926 m 361.879 336.926 l 361.879 336.926 m 409.765
311.748 l 409.765 311.748 m 409.765 311.748 l 409.765 311.748 m
409.765 311.748 l 409.765 311.748 m 475.121 346.112 l 475.121
346.112 m 475.121 346.112 l 475.121 346.112 m 475.121 346.112 l
475.121 346.112 m 432.629 368.454 l 432.629 368.454 m 432.629
368.454 l 432.629 368.454 m 432.629 368.454 l 432.629 368.454 m
498.429 403.052 l 498.429 403.052 m 498.429 403.052 l 498.429
403.052 m 498.429 403.052 l 498.429 403.052 m 545.871 378.107 l
545.871 378.107 m 545.871 378.107 l 545.871 378.107 m 545.871
378.107 l 545.871 378.107 m 490.414 348.948 l 490.414 348.948 m
490.414 348.948 l 490.414 348.948 m 490.414 348.948 l 490.414
348.948 m 432.629 379.331 l stroke 432.629 379.331 m 432.629 379.331
l 432.629 379.331 m 432.629 379.331 l 432.629 379.331 m 477.744
403.052 l 477.744 403.052 m 477.744 403.052 l 477.744 403.052 m
477.744 403.052 l 477.744 403.052 m 545.871 367.231 l 545.871
367.231 m 545.871 367.231 l 545.871 367.231 m 545.871 367.231 l
545.871 367.231 m 503.379 344.888 l 503.379 344.888 m 503.379
344.888 l 503.379 344.888 m 503.379 344.888 l 503.379 344.888 m
566.408 311.748 l 566.408 311.748 m 566.408 311.748 l 566.408
311.748 m 566.408 311.748 l 566.408 311.748 m 616.621 338.150 l
616.621 338.150 m 616.621 338.150 l 616.621 338.150 m 616.621
338.150 l 616.621 338.150 m 563.935 365.852 l 563.935 365.852 m
563.935 365.852 l 563.935 365.852 m 563.935 365.852 l 563.935
365.852 m 503.379 334.012 l 503.379 334.012 m 503.379 334.012 l
503.379 334.012 m 503.379 334.012 l 503.379 334.012 m 545.871
311.669 l 545.871 311.669 m 545.871 311.669 l 545.871 311.669 m
545.871 311.669 l 545.871 311.669 m 475.271 274.548 l 475.271
274.548 m 475.271 274.548 l 475.271 274.548 m 475.271 274.548 l
475.271 274.548 m 432.629 296.969 l 432.629 296.969 m 432.629
296.969 l 432.629 296.969 m 432.629 296.969 l 432.629 296.969 m
492.887 328.652 l 492.887 328.652 m 492.887 328.652 l 492.887
328.652 m 492.887 328.652 l 492.887 328.652 m 545.871 300.793 l
545.871 300.793 m 545.871 300.793 l 545.871 300.793 m 545.871
300.793 l 545.871 300.793 m 495.956 274.548 l 495.956 274.548 m
495.956 274.548 l 495.956 274.548 m 495.956 274.548 l 495.956
274.548 m 432.629 307.845 l 432.629 307.845 m 432.629 307.845 l
432.629 307.845 m 432.629 307.845 l 432.629 307.845 m 475.121
330.188 l 475.121 330.188 m 475.121 330.188 l 475.121 330.188 m
475.121 330.188 l 475.121 330.188 m 407.292 365.852 l 407.292
365.852 m 407.292 365.852 l 407.292 365.852 m 407.292 365.852 l
407.292 365.852 m 361.879 341.974 l 361.879 341.974 m 361.879
341.974 l 361.879 341.974 m 361.879 341.974 l 361.879 341.974 m
419.365 311.748 l 419.365 311.748 m 419.365 311.748 l 419.365
311.748 m 419.365 311.748 l 419.365 311.748 m 475.121 341.064 l
475.121 341.064 m 475.121 341.064 l 475.121 341.064 m 475.121
341.064 l 475.121 341.064 m 427.978 365.852 l 427.978 365.852 m
427.978 365.852 l 427.978 365.852 m 427.978 365.852 l 427.978
365.852 m 361.879 331.098 l 361.879 331.098 m 361.879 331.098 l
361.879 331.098 m 361.879 331.098 l 361.879 331.098 m 404.371
308.755 l 404.371 308.755 m 404.371 308.755 l 404.371 308.755 m
404.371 308.755 l 404.371 308.755 m 339.313 274.548 l 339.313
274.548 m 339.313 274.548 l 339.313 274.548 m 339.313 274.548 l
339.313 274.548 m 291.129 299.883 l 291.129 299.883 m 291.129
299.883 l 291.129 299.883 m 291.129 299.883 l 291.129 299.883 m
345.844 328.652 l 345.844 328.652 m 345.844 328.652 l 345.844
328.652 m 345.844 328.652 l 345.844 328.652 m 404.371 297.879 l
404.371 297.879 m 404.371 297.879 l 404.371 297.879 m 404.371
297.879 l 404.371 297.879 m 359.999 274.548 l 359.999 274.548 m
359.999 274.548 l 359.999 274.548 m 359.999 274.548 l 359.999
274.548 m 291.129 310.760 l 291.129 310.760 m 291.129 310.760 l
291.129 310.760 m 291.129 310.760 l 291.129 310.760 m 333.621
333.102 l 333.621 333.102 m 333.621 333.102 l 333.621 333.102 m
333.621 333.102 l 333.621 333.102 m 271.335 365.852 l 271.335
365.852 m 271.335 365.852 l 271.335 365.852 m 271.335 365.852 l
271.335 365.852 m 220.379 339.060 l 220.379 339.060 m 220.379
339.060 l 220.379 339.060 m 220.379 339.060 l 220.379 339.060 m
272.322 311.748 l 272.322 311.748 m 272.322 311.748 l 272.322
311.748 m 272.322 311.748 l 272.322 311.748 m 333.621 343.979 l
333.621 343.979 m 333.621 343.979 l 333.621 343.979 m 333.621
343.979 l 333.621 343.979 m 291.129 366.321 l 291.129 366.321 m
291.129 366.321 l 291.129 366.321 m 291.129 366.321 l 291.129
366.321 m 360.987 403.052 l 360.987 403.052 m 360.987 403.052 l
360.987 403.052 m 360.987 403.052 l 360.987 403.052 m 404.371
380.241 l 404.371 380.241 m 404.371 380.241 l 404.371 380.241 m
404.371 380.241 l 404.371 380.241 m 344.856 348.948 l 344.856
348.948 m 344.856 348.948 l 344.856 348.948 m 344.856 348.948 l
344.856 348.948 m 291.129 377.197 l 291.129 377.197 m 291.129
377.197 l 291.129 377.197 m 291.129 377.197 l 291.129 377.197 m
340.301 403.052 l 340.301 403.052 m 340.301 403.052 l 340.301
403.052 m 340.301 403.052 l 340.301 403.052 m 404.371 369.364 l
404.371 369.364 m 404.371 369.364 l 404.371 369.364 m 404.371
369.364 l 404.371 369.364 m 361.879 347.022 l 361.879 347.022 m
361.879 347.022 l 361.879 347.022 m 361.879 347.022 l 361.879
347.022 m 428.965 311.748 l 428.965 311.748 m 428.965 311.748 l
428.965 311.748 m 428.965 311.748 l 428.965 311.748 m 475.121
336.016 l 475.121 336.016 m 475.121 336.016 l 475.121 336.016 m
475.121 336.016 l 475.121 336.016 m 418.377 365.852 l 418.377
365.852 m 418.377 365.852 l 418.377 365.852 m 418.377 365.852 l
418.377 365.852 m 361.879 336.145 l 361.879 336.145 m 361.879
336.145 l 361.879 336.145 m 361.879 336.145 l 361.879 336.145 m
408.280 311.748 l 408.280 311.748 m 408.280 311.748 l 408.280
311.748 m 408.280 311.748 l 408.280 311.748 m 475.121 346.893 l
475.121 346.893 m 475.121 346.893 l 475.121 346.893 m 475.121
346.893 l 475.121 346.893 m 432.629 369.235 l 432.629 369.235 m
432.629 369.235 l 432.629 369.235 m 432.629 369.235 l 432.629
369.235 m 496.944 403.052 l 496.944 403.052 m 496.944 403.052 l
496.944 403.052 m 496.944 403.052 l 496.944 403.052 m 545.871
377.326 l 545.871 377.326 m 545.871 377.326 l 545.871 377.326 m
545.871 377.326 l 545.871 377.326 m 491.899 348.948 l 491.899
348.948 m 491.899 348.948 l 491.899 348.948 m 491.899 348.948 l
491.899 348.948 m 432.629 380.112 l 432.629 380.112 m 432.629
380.112 l 432.629 380.112 m 432.629 380.112 l 432.629 380.112 m
476.258 403.052 l 476.258 403.052 m 476.258 403.052 l 476.258
403.052 m 476.258 403.052 l 476.258 403.052 m 545.871 366.450 l
545.871 366.450 m 545.871 366.450 l 545.871 366.450 m 545.871
366.450 l 545.871 366.450 m 503.379 344.107 l 503.379 344.107 m
503.379 344.107 l 503.379 344.107 m 503.379 344.107 l 503.379
344.107 m 564.923 311.748 l 564.923 311.748 m 564.923 311.748 l
564.923 311.748 m 564.923 311.748 l 564.923 311.748 m 616.621
338.931 l 616.621 338.931 m 616.621 338.931 l 616.621 338.931 m
616.621 338.931 l 616.621 338.931 m 565.420 365.852 l 565.420
365.852 m 565.420 365.852 l 565.420 365.852 m 565.420 365.852 l
565.420 365.852 m 503.379 333.231 l 503.379 333.231 m 503.379
333.231 l 503.379 333.231 m 503.379 333.231 l 503.379 333.231 m
545.871 310.889 l 545.871 310.889 m 545.871 310.889 l 545.871
310.889 m 545.871 310.889 l 545.871 310.889 m 476.756 274.548 l
476.756 274.548 m 476.756 274.548 l 476.756 274.548 m 476.756
274.548 l 476.756 274.548 m 432.629 297.750 l 432.629 297.750 m
432.629 297.750 l 432.629 297.750 m 432.629 297.750 l 432.629
297.750 m 491.401 328.652 l 491.401 328.652 m 491.401 328.652 l
491.401 328.652 m 491.401 328.652 l 491.401 328.652 m 545.871
300.012 l 545.871 300.012 m 545.871 300.012 l 545.871 300.012 m
545.871 300.012 l 545.871 300.012 m 497.441 274.548 l 497.441
274.548 m 497.441 274.548 l 497.441 274.548 m 497.441 274.548 l
497.441 274.548 m 432.629 308.626 l 432.629 308.626 m 432.629
308.626 l 432.629 308.626 m 432.629 308.626 l 432.629 308.626 m
475.121 330.969 l 475.121 330.969 m 475.121 330.969 l 475.121
330.969 m 475.121 330.969 l 475.121 330.969 m 408.777 365.852 l
408.777 365.852 m 408.777 365.852 l 408.777 365.852 m 408.777
365.852 l 408.777 365.852 m 361.879 341.193 l 361.879 341.193 m
361.879 341.193 l 361.879 341.193 m 361.879 341.193 l 361.879
341.193 m 417.880 311.748 l 417.880 311.748 m 417.880 311.748 l
417.880 311.748 m 417.880 311.748 l 417.880 311.748 m 475.121
341.845 l 475.121 341.845 m 475.121 341.845 l 475.121 341.845 m
475.121 341.845 l 475.121 341.845 m 429.463 365.852 l 429.463
365.852 m 429.463 365.852 l 429.463 365.852 m 429.463 365.852 l
429.463 365.852 m 361.879 330.317 l 361.879 330.317 m 361.879
330.317 l 361.879 330.317 m 361.879 330.317 l 361.879 330.317 m
404.371 307.974 l 404.371 307.974 m 404.371 307.974 l 404.371
307.974 m 404.371 307.974 l 404.371 307.974 m 340.798 274.548 l
340.798 274.548 m 340.798 274.548 l 340.798 274.548 m 340.798
274.548 l 340.798 274.548 m 291.129 300.664 l 291.129 300.664 m
291.129 300.664 l 291.129 300.664 m 291.129 300.664 l 291.129
300.664 m 344.359 328.652 l 344.359 328.652 m 344.359 328.652 l
344.359 328.652 m 344.359 328.652 l 344.359 328.652 m 404.371
297.098 l 404.371 297.098 m 404.371 297.098 l 404.371 297.098 m
404.371 297.098 l 404.371 297.098 m 361.484 274.548 l 361.484
274.548 m 361.484 274.548 l 361.484 274.548 m 361.484 274.548 l
361.484 274.548 m 291.129 311.540 l 291.129 311.540 m 291.129
311.540 l 291.129 311.540 m 291.129 311.540 l 291.129 311.540 m
333.621 333.883 l 333.621 333.883 m 333.621 333.883 l 333.621
333.883 m 333.621 333.883 l 333.621 333.883 m 272.820 365.852 l
272.820 365.852 m 272.820 365.852 l 272.820 365.852 m 272.820
365.852 l 272.820 365.852 m 220.379 338.279 l 220.379 338.279 m
220.379 338.279 l 220.379 338.279 m 220.379 338.279 l stroke 220.379
338.279 m 270.837 311.748 l 270.837 311.748 m 270.837 311.748 l
270.837 311.748 m 270.837 311.748 l 270.837 311.748 m 333.621
344.759 l 333.621 344.759 m 333.621 344.759 l 333.621 344.759 m
333.621 344.759 l 333.621 344.759 m 291.129 367.102 l 291.129
367.102 m 291.129 367.102 l 291.129 367.102 m 291.129 367.102 l
291.129 367.102 m 359.502 403.052 l 359.502 403.052 m 359.502
403.052 l 359.502 403.052 m 359.502 403.052 l 359.502 403.052 m
404.371 379.460 l 404.371 379.460 m 404.371 379.460 l 404.371
379.460 m 404.371 379.460 l 404.371 379.460 m 346.341 348.948 l
346.341 348.948 m 346.341 348.948 l 346.341 348.948 m 346.341
348.948 l 346.341 348.948 m 291.129 377.978 l 291.129 377.978 m
291.129 377.978 l 291.129 377.978 m 291.129 377.978 l 291.129
377.978 m 338.816 403.052 l 338.816 403.052 m 338.816 403.052 l
338.816 403.052 m 338.816 403.052 l 338.816 403.052 m 404.371
368.583 l 404.371 368.583 m 404.371 368.583 l 404.371 368.583 m
404.371 368.583 l 404.371 368.583 m 361.879 346.241 l 361.879
346.241 m 361.879 346.241 l 361.879 346.241 m 361.879 346.241 l
361.879 346.241 m 427.480 311.748 l 427.480 311.748 m 427.480
311.748 l 427.480 311.748 m 427.480 311.748 l 427.480 311.748 m
475.121 336.797 l 475.121 336.797 m 475.121 336.797 l 475.121
336.797 m 475.121 336.797 l 475.121 336.797 m 419.863 365.852 l
419.863 365.852 m 419.863 365.852 l 419.863 365.852 m 419.863
365.852 l 419.863 365.852 m 361.879 335.364 l 361.879 335.364 m
361.879 335.364 l 361.879 335.364 m 361.879 335.364 l 361.879
335.364 m 406.795 311.748 l 406.795 311.748 m 406.795 311.748 l
406.795 311.748 m 406.795 311.748 l 406.795 311.748 m 475.121
347.674 l 475.121 347.674 m 475.121 347.674 l 475.121 347.674 m
475.121 347.674 l 475.121 347.674 m 432.629 370.016 l 432.629
370.016 m 432.629 370.016 l 432.629 370.016 m 432.629 370.016 l
432.629 370.016 m 495.459 403.052 l 495.459 403.052 m 495.459
403.052 l 495.459 403.052 m 495.459 403.052 l 495.459 403.052 m
545.871 376.546 l 545.871 376.546 m 545.871 376.546 l 545.871
376.546 m 545.871 376.546 l 545.871 376.546 m 493.384 348.948 l
493.384 348.948 m 493.384 348.948 l 493.384 348.948 m 493.384
348.948 l 493.384 348.948 m 432.629 380.893 l 432.629 380.893 m
432.629 380.893 l 432.629 380.893 m 432.629 380.893 l 432.629
380.893 m 475.121 403.235 l 475.121 403.235 m 475.121 403.235 l
475.121 403.235 m 475.121 403.235 l 475.121 403.235 m 404.720
440.252 l 404.720 440.252 m 404.720 440.252 l 404.720 440.252 m
404.720 440.252 l 404.720 440.252 m 361.879 417.727 l 361.879
417.727 m 361.879 417.727 l 361.879 417.727 m 361.879 417.727 l
361.879 417.727 m 421.938 386.148 l 421.938 386.148 m 421.938
386.148 l 421.938 386.148 m 421.938 386.148 l 421.938 386.148 m
475.121 414.112 l 475.121 414.112 m 475.121 414.112 l 475.121
414.112 m 475.121 414.112 l 475.121 414.112 m 425.405 440.252 l
425.405 440.252 m 425.405 440.252 l 425.405 440.252 m 425.405
440.252 l 425.405 440.252 m 361.879 406.850 l 361.879 406.850 m
361.879 406.850 l 361.879 406.850 m 361.879 406.850 l 361.879
406.850 m 404.371 384.508 l 404.371 384.508 m 404.371 384.508 l
404.371 384.508 m 404.371 384.508 l 404.371 384.508 m 336.741
348.948 l 336.741 348.948 m 336.741 348.948 l 336.741 348.948 m
336.741 348.948 l 336.741 348.948 m 291.129 372.931 l 291.129
372.931 m 291.129 372.931 l 291.129 372.931 m 291.129 372.931 l
291.129 372.931 m 348.416 403.052 l 348.416 403.052 m 348.416
403.052 l 348.416 403.052 m 348.416 403.052 l 348.416 403.052 m
404.371 373.631 l 404.371 373.631 m 404.371 373.631 l 404.371
373.631 m 404.371 373.631 l 404.371 373.631 m 357.427 348.948 l
357.427 348.948 m 357.427 348.948 l 357.427 348.948 m 357.427
348.948 l 357.427 348.948 m 291.129 383.807 l 291.129 383.807 m
291.129 383.807 l 291.129 383.807 m 291.129 383.807 l 291.129
383.807 m 333.621 406.150 l 333.621 406.150 m 333.621 406.150 l
333.621 406.150 m 333.621 406.150 l 333.621 406.150 m 268.762
440.252 l 268.762 440.252 m 268.762 440.252 l 268.762 440.252 m
268.762 440.252 l 268.762 440.252 m 220.379 414.812 l 220.379
414.812 m 220.379 414.812 l 220.379 414.812 m 220.379 414.812 l
220.379 414.812 m 274.895 386.148 l 274.895 386.148 m 274.895
386.148 l 274.895 386.148 m 274.895 386.148 l 274.895 386.148 m
333.621 417.026 l 333.621 417.026 m 333.621 417.026 l 333.621
417.026 m 333.621 417.026 l 333.621 417.026 m 289.448 440.252 l
289.448 440.252 m 289.448 440.252 l 289.448 440.252 m 289.448
440.252 l 289.448 440.252 m 220.379 403.936 l 220.379 403.936 m
220.379 403.936 l 220.379 403.936 m 220.379 403.936 l 220.379
403.936 m 262.871 381.593 l 262.871 381.593 m 262.871 381.593 l
262.871 381.593 m 262.871 381.593 l 262.871 381.593 m 200.784
348.948 l 200.784 348.948 m 200.784 348.948 l 200.784 348.948 m
200.784 348.948 l 200.784 348.948 m 149.629 375.845 l 149.629
375.845 m 149.629 375.845 l 149.629 375.845 m 149.629 375.845 l
149.629 375.845 m 201.374 403.052 l 201.374 403.052 m 201.374
403.052 l 201.374 403.052 m 201.374 403.052 l 201.374 403.052 m
262.871 370.717 l 262.871 370.717 m 262.871 370.717 l 262.871
370.717 m 262.871 370.717 l 262.871 370.717 m 220.379 348.374 l
220.379 348.374 m 220.379 348.374 l 220.379 348.374 m 220.379
348.374 l 220.379 348.374 m 290.038 311.748 l 290.038 311.748 m
290.038 311.748 l 290.038 311.748 m 290.038 311.748 l 290.038
311.748 m 333.621 334.664 l 333.621 334.664 m 333.621 334.664 l
333.621 334.664 m 333.621 334.664 l 333.621 334.664 m 274.305
365.852 l 274.305 365.852 m 274.305 365.852 l 274.305 365.852 m
274.305 365.852 l 274.305 365.852 m 220.379 337.498 l 220.379
337.498 m 220.379 337.498 l 220.379 337.498 m 220.379 337.498 l
220.379 337.498 m 269.352 311.748 l 269.352 311.748 m 269.352
311.748 l 269.352 311.748 m 269.352 311.748 l 269.352 311.748 m
333.621 345.540 l 333.621 345.540 m 333.621 345.540 l 333.621
345.540 m 333.621 345.540 l 333.621 345.540 m 291.129 367.883 l
291.129 367.883 m 291.129 367.883 l 291.129 367.883 m 291.129
367.883 l 291.129 367.883 m 358.017 403.052 l 358.017 403.052 m
358.017 403.052 l 358.017 403.052 m 358.017 403.052 l 358.017
403.052 m 404.371 378.679 l 404.371 378.679 m 404.371 378.679 l
404.371 378.679 m 404.371 378.679 l 404.371 378.679 m 347.826
348.948 l 347.826 348.948 m 347.826 348.948 l 347.826 348.948 m
347.826 348.948 l 347.826 348.948 m 291.129 378.759 l 291.129
378.759 m 291.129 378.759 l 291.129 378.759 m 291.129 378.759 l
291.129 378.759 m 337.331 403.052 l 337.331 403.052 m 337.331
403.052 l 337.331 403.052 m 337.331 403.052 l 337.331 403.052 m
404.371 367.803 l 404.371 367.803 m 404.371 367.803 l 404.371
367.803 m 404.371 367.803 l 404.371 367.803 m 361.879 345.460 l
361.879 345.460 m 361.879 345.460 l 361.879 345.460 m 361.879
345.460 l 361.879 345.460 m 425.995 311.748 l 425.995 311.748 m
425.995 311.748 l 425.995 311.748 m 425.995 311.748 l 425.995
311.748 m 475.121 337.578 l 475.121 337.578 m 475.121 337.578 l
475.121 337.578 m 475.121 337.578 l 475.121 337.578 m 421.348
365.852 l 421.348 365.852 m 421.348 365.852 l 421.348 365.852 m
421.348 365.852 l 421.348 365.852 m 361.879 334.584 l 361.879
334.584 m 361.879 334.584 l 361.879 334.584 m 361.879 334.584 l
361.879 334.584 m 405.309 311.748 l 405.309 311.748 m 405.309
311.748 l 405.309 311.748 m 405.309 311.748 l 405.309 311.748 m
475.121 348.455 l 475.121 348.455 m 475.121 348.455 l 475.121
348.455 m 475.121 348.455 l 475.121 348.455 m 432.629 370.797 l
432.629 370.797 m 432.629 370.797 l 432.629 370.797 m 432.629
370.797 l 432.629 370.797 m 493.974 403.052 l 493.974 403.052 m
493.974 403.052 l 493.974 403.052 m 493.974 403.052 l 493.974
403.052 m 545.871 375.765 l 545.871 375.765 m 545.871 375.765 l
545.871 375.765 m 545.871 375.765 l 545.871 375.765 m 494.869
348.948 l 494.869 348.948 m 494.869 348.948 l 494.869 348.948 m
494.869 348.948 l 494.869 348.948 m 432.629 381.674 l 432.629
381.674 m 432.629 381.674 l 432.629 381.674 m 432.629 381.674 l
432.629 381.674 m 475.121 404.016 l 475.121 404.016 m 475.121
404.016 l 475.121 404.016 m 475.121 404.016 l 475.121 404.016 m
406.205 440.252 l 406.205 440.252 m 406.205 440.252 l 406.205
440.252 m 406.205 440.252 l 406.205 440.252 m 361.879 416.946 l
361.879 416.946 m 361.879 416.946 l 361.879 416.946 m 361.879
416.946 l 361.879 416.946 m 420.452 386.148 l 420.452 386.148 m
420.452 386.148 l 420.452 386.148 m 420.452 386.148 l 420.452
386.148 m 475.121 414.893 l 475.121 414.893 m 475.121 414.893 l
475.121 414.893 m 475.121 414.893 l 475.121 414.893 m 426.890
440.252 l 426.890 440.252 m 426.890 440.252 l 426.890 440.252 m
426.890 440.252 l 426.890 440.252 m 361.879 406.069 l 361.879
406.069 m 361.879 406.069 l 361.879 406.069 m 361.879 406.069 l
361.879 406.069 m 404.371 383.727 l 404.371 383.727 m 404.371
383.727 l 404.371 383.727 m 404.371 383.727 l 404.371 383.727 m
338.226 348.948 l 338.226 348.948 m 338.226 348.948 l 338.226
348.948 m 338.226 348.948 l 338.226 348.948 m 291.129 373.711 l
291.129 373.711 m 291.129 373.711 l 291.129 373.711 m 291.129
373.711 l 291.129 373.711 m 346.931 403.052 l 346.931 403.052 m
346.931 403.052 l stroke 346.931 403.052 m 346.931 403.052 l 346.931
403.052 m 404.371 372.850 l 404.371 372.850 m 404.371 372.850 l
404.371 372.850 m 404.371 372.850 l 404.371 372.850 m 358.912
348.948 l 358.912 348.948 m 358.912 348.948 l 358.912 348.948 m
358.912 348.948 l 358.912 348.948 m 291.129 384.588 l 291.129
384.588 m 291.129 384.588 l 291.129 384.588 m 291.129 384.588 l
291.129 384.588 m 333.621 406.930 l 333.621 406.930 m 333.621
406.930 l 333.621 406.930 m 333.621 406.930 l 333.621 406.930 m
270.247 440.252 l 270.247 440.252 m 270.247 440.252 l 270.247
440.252 m 270.247 440.252 l 270.247 440.252 m 220.379 414.031 l
220.379 414.031 m 220.379 414.031 l 220.379 414.031 m 220.379
414.031 l 220.379 414.031 m 273.410 386.148 l 273.410 386.148 m
273.410 386.148 l 273.410 386.148 m 273.410 386.148 l 273.410
386.148 m 333.621 417.807 l 333.621 417.807 m 333.621 417.807 l
333.621 417.807 m 333.621 417.807 l 333.621 417.807 m 290.933
440.252 l 290.933 440.252 m 290.933 440.252 l 290.933 440.252 m
290.933 440.252 l 290.933 440.252 m 220.379 403.155 l 220.379
403.155 m 220.379 403.155 l 220.379 403.155 m 220.379 403.155 l
220.379 403.155 m 262.871 380.812 l 262.871 380.812 m 262.871
380.812 l 262.871 380.812 m 262.871 380.812 l 262.871 380.812 m
202.269 348.948 l 202.269 348.948 m 202.269 348.948 l 202.269
348.948 m 202.269 348.948 l 202.269 348.948 m 149.629 376.626 l
149.629 376.626 m 149.629 376.626 l 149.629 376.626 m 149.629
376.626 l 149.629 376.626 m 199.888 403.052 l 199.888 403.052 m
199.888 403.052 l 199.888 403.052 m 199.888 403.052 l 199.888
403.052 m 262.871 369.936 l 262.871 369.936 m 262.871 369.936 l
262.871 369.936 m 262.871 369.936 l 262.871 369.936 m 220.379
347.593 l 220.379 347.593 m 220.379 347.593 l 220.379 347.593 m
220.379 347.593 l 220.379 347.593 m 288.553 311.748 l 288.553
311.748 m 288.553 311.748 l 288.553 311.748 m 288.553 311.748 l
288.553 311.748 m 333.621 335.445 l 333.621 335.445 m 333.621
335.445 l 333.621 335.445 m 333.621 335.445 l 333.621 335.445 m
275.790 365.852 l 275.790 365.852 m 275.790 365.852 l 275.790
365.852 m 275.790 365.852 l 275.790 365.852 m 220.379 336.717 l
220.379 336.717 m 220.379 336.717 l 220.379 336.717 m 220.379
336.717 l 220.379 336.717 m 267.867 311.748 l 267.867 311.748 m
267.867 311.748 l 267.867 311.748 m 267.867 311.748 l 267.867
311.748 m 333.621 346.321 l 333.621 346.321 m 333.621 346.321 l
333.621 346.321 m 333.621 346.321 l 333.621 346.321 m 291.129
368.664 l 291.129 368.664 m 291.129 368.664 l 291.129 368.664 m
291.129 368.664 l 291.129 368.664 m 356.531 403.052 l 356.531
403.052 m 356.531 403.052 l 356.531 403.052 m 356.531 403.052 l
356.531 403.052 m 404.371 377.898 l 404.371 377.898 m 404.371
377.898 l 404.371 377.898 m 404.371 377.898 l 404.371 377.898 m
349.312 348.948 l 349.312 348.948 m 349.312 348.948 l 349.312
348.948 m 349.312 348.948 l 349.312 348.948 m 291.129 379.540 l
291.129 379.540 m 291.129 379.540 l 291.129 379.540 m 291.129
379.540 l 291.129 379.540 m 335.846 403.052 l 335.846 403.052 m
335.846 403.052 l 335.846 403.052 m 335.846 403.052 l 335.846
403.052 m 404.371 367.022 l 404.371 367.022 m 404.371 367.022 l
404.371 367.022 m 404.371 367.022 l 404.371 367.022 m 361.879
344.679 l 361.879 344.679 m 361.879 344.679 l 361.879 344.679 m
361.879 344.679 l 361.879 344.679 m 424.510 311.748 l 424.510
311.748 m 424.510 311.748 l 424.510 311.748 m 424.510 311.748 l
424.510 311.748 m 475.121 338.359 l 475.121 338.359 m 475.121
338.359 l 475.121 338.359 m 475.121 338.359 l 475.121 338.359 m
422.833 365.852 l 422.833 365.852 m 422.833 365.852 l 422.833
365.852 m 422.833 365.852 l 422.833 365.852 m 361.879 333.803 l
361.879 333.803 m 361.879 333.803 l 361.879 333.803 m 361.879
333.803 l 361.879 333.803 m 404.371 311.460 l 404.371 311.460 m
404.371 311.460 l 404.371 311.460 m 404.371 311.460 l 404.371
311.460 m 334.169 274.548 l 334.169 274.548 m 334.169 274.548 l
334.169 274.548 m 334.169 274.548 l 334.169 274.548 m 291.129
297.178 l 291.129 297.178 m 291.129 297.178 l 291.129 297.178 m
291.129 297.178 l 291.129 297.178 m 350.989 328.652 l 350.989
328.652 m 350.989 328.652 l 350.989 328.652 m 350.989 328.652 l
350.989 328.652 m 404.371 300.584 l 404.371 300.584 m 404.371
300.584 l 404.371 300.584 m 404.371 300.584 l 404.371 300.584 m
354.854 274.548 l 354.854 274.548 m 354.854 274.548 l 354.854
274.548 m 354.854 274.548 l 354.854 274.548 m 291.129 308.054 l
291.129 308.054 m 291.129 308.054 l 291.129 308.054 m 291.129
308.054 l 291.129 308.054 m 333.621 330.397 l 333.621 330.397 m
333.621 330.397 l 333.621 330.397 m 333.621 330.397 l 333.621
330.397 m 266.190 365.852 l 266.190 365.852 m 266.190 365.852 l
266.190 365.852 m 266.190 365.852 l 266.190 365.852 m 220.379
341.765 l 220.379 341.765 m 220.379 341.765 l 220.379 341.765 m
220.379 341.765 l 220.379 341.765 m 277.467 311.748 l 277.467
311.748 m 277.467 311.748 l 277.467 311.748 m 277.467 311.748 l
277.467 311.748 m 333.621 341.273 l 333.621 341.273 m 333.621
341.273 l 333.621 341.273 m 333.621 341.273 l 333.621 341.273 m
286.876 365.852 l 286.876 365.852 m 286.876 365.852 l 286.876
365.852 m 286.876 365.852 l 286.876 365.852 m 220.379 330.888 l
220.379 330.888 m 220.379 330.888 l 220.379 330.888 m 220.379
330.888 l 220.379 330.888 m 262.871 308.546 l 262.871 308.546 m
262.871 308.546 l 262.871 308.546 m 262.871 308.546 l 262.871
308.546 m 198.211 274.548 l 198.211 274.548 m 198.211 274.548 l
198.211 274.548 m 198.211 274.548 l 198.211 274.548 m 149.629
300.092 l 149.629 300.092 m 149.629 300.092 l 149.629 300.092 m
149.629 300.092 l 149.629 300.092 m 203.946 328.652 l 203.946
328.652 m 203.946 328.652 l 203.946 328.652 m 203.946 328.652 l
203.946 328.652 m 262.871 297.669 l 262.871 297.669 m 262.871
297.669 l 262.871 297.669 m 262.871 297.669 l 262.871 297.669 m
218.897 274.548 l 218.897 274.548 m 218.897 274.548 l 218.897
274.548 m 218.897 274.548 l 218.897 274.548 m 149.629 310.969 l
149.629 310.969 m 149.629 310.969 l 149.629 310.969 m 149.629
310.969 l 149.629 310.969 m 192.121 333.311 l 192.121 333.311 m
192.121 333.311 l 192.121 333.311 m 192.121 333.311 l 192.121
333.311 m 130.233 365.852 l 130.233 365.852 m 130.233 365.852 l
130.233 365.852 m 130.233 365.852 l 130.233 365.852 m 78.879 338.850
l 78.879 338.850 m 78.879 338.850 l 78.879 338.850 m 78.879 338.850
l 78.879 338.850 m 130.425 311.748 l 130.425 311.748 m 130.425
311.748 l 130.425 311.748 m 130.425 311.748 l 130.425 311.748 m
192.121 344.188 l 192.121 344.188 m 192.121 344.188 l 192.121
344.188 m 192.121 344.188 l 192.121 344.188 m 149.629 366.530 l
149.629 366.530 m 149.629 366.530 l 149.629 366.530 m 149.629
366.530 l 149.629 366.530 m 219.089 403.052 l 219.089 403.052 m
219.089 403.052 l 219.089 403.052 m 219.089 403.052 l 219.089
403.052 m 262.871 380.032 l 262.871 380.032 m 262.871 380.032 l
262.871 380.032 m 262.871 380.032 l 262.871 380.032 m 203.754
348.948 l 203.754 348.948 m 203.754 348.948 l 203.754 348.948 m
203.754 348.948 l 203.754 348.948 m 149.629 377.407 l 149.629
377.407 m 149.629 377.407 l 149.629 377.407 m 149.629 377.407 l
149.629 377.407 m 198.403 403.052 l 198.403 403.052 m 198.403
403.052 l 198.403 403.052 m 198.403 403.052 l 198.403 403.052 m
262.871 369.155 l 262.871 369.155 m 262.871 369.155 l 262.871
369.155 m 262.871 369.155 l 262.871 369.155 m 220.379 346.813 l
220.379 346.813 m 220.379 346.813 l 220.379 346.813 m 220.379
346.813 l 220.379 346.813 m 287.068 311.748 l 287.068 311.748 m
287.068 311.748 l 287.068 311.748 m 287.068 311.748 l 287.068
311.748 m 333.621 336.226 l 333.621 336.226 m 333.621 336.226 l
333.621 336.226 m 333.621 336.226 l 333.621 336.226 m 277.275
365.852 l 277.275 365.852 m 277.275 365.852 l 277.275 365.852 m
277.275 365.852 l 277.275 365.852 m 220.379 335.936 l 220.379
335.936 m 220.379 335.936 l 220.379 335.936 m 220.379 335.936 l
220.379 335.936 m 266.382 311.748 l 266.382 311.748 m 266.382
311.748 l 266.382 311.748 m 266.382 311.748 l 266.382 311.748 m
333.621 347.102 l 333.621 347.102 m 333.621 347.102 l 333.621
347.102 m 333.621 347.102 l 333.621 347.102 m 291.129 369.445 l
291.129 369.445 m 291.129 369.445 l 291.129 369.445 m 291.129
369.445 l 291.129 369.445 m 355.046 403.052 l 355.046 403.052 m
355.046 403.052 l 355.046 403.052 m 355.046 403.052 l 355.046
403.052 m 404.371 377.117 l 404.371 377.117 m 404.371 377.117 l
404.371 377.117 m 404.371 377.117 l 404.371 377.117 m 350.797
348.948 l 350.797 348.948 m 350.797 348.948 l 350.797 348.948 m
350.797 348.948 l 350.797 348.948 m 291.129 380.321 l 291.129
380.321 m 291.129 380.321 l 291.129 380.321 m 291.129 380.321 l
291.129 380.321 m 334.360 403.052 l 334.360 403.052 m 334.360
403.052 l 334.360 403.052 m 334.360 403.052 l 334.360 403.052 m
404.371 366.241 l 404.371 366.241 m 404.371 366.241 l 404.371
366.241 m 404.371 366.241 l 404.371 366.241 m 361.879 343.898 l
361.879 343.898 m 361.879 343.898 l 361.879 343.898 m 361.879
343.898 l 361.879 343.898 m 423.025 311.748 l 423.025 311.748 m
423.025 311.748 l 423.025 311.748 m 423.025 311.748 l 423.025
311.748 m 475.121 339.140 l stroke 475.121 339.140 m 475.121 339.140
l 475.121 339.140 m 475.121 339.140 l 475.121 339.140 m 424.318
365.852 l 424.318 365.852 m 424.318 365.852 l 424.318 365.852 m
424.318 365.852 l 424.318 365.852 m 361.879 333.022 l 361.879
333.022 m 361.879 333.022 l 361.879 333.022 m 361.879 333.022 l
361.879 333.022 m 404.371 310.679 l 404.371 310.679 m 404.371
310.679 l 404.371 310.679 m 404.371 310.679 l 404.371 310.679 m
335.654 274.548 l 335.654 274.548 m 335.654 274.548 l 335.654
274.548 m 335.654 274.548 l 335.654 274.548 m 291.129 297.959 l
291.129 297.959 m 291.129 297.959 l 291.129 297.959 m 291.129
297.959 l 291.129 297.959 m 349.503 328.652 l 349.503 328.652 m
349.503 328.652 l 349.503 328.652 m 349.503 328.652 l 349.503
328.652 m 404.371 299.803 l 404.371 299.803 m 404.371 299.803 l
404.371 299.803 m 404.371 299.803 l 404.371 299.803 m 356.339
274.548 l 356.339 274.548 m 356.339 274.548 l 356.339 274.548 m
356.339 274.548 l 356.339 274.548 m 291.129 308.835 l 291.129
308.835 m 291.129 308.835 l 291.129 308.835 m 291.129 308.835 l
291.129 308.835 m 333.621 331.178 l 333.621 331.178 m 333.621
331.178 l 333.621 331.178 m 333.621 331.178 l 333.621 331.178 m
267.675 365.852 l 267.675 365.852 m 267.675 365.852 l 267.675
365.852 m 267.675 365.852 l 267.675 365.852 m 220.379 340.984 l
220.379 340.984 m 220.379 340.984 l 220.379 340.984 m 220.379
340.984 l 220.379 340.984 m 275.982 311.748 l 275.982 311.748 m
275.982 311.748 l 275.982 311.748 m 275.982 311.748 l 275.982
311.748 m 333.621 342.054 l 333.621 342.054 m 333.621 342.054 l
333.621 342.054 m 333.621 342.054 l 333.621 342.054 m 288.361
365.852 l 288.361 365.852 m 288.361 365.852 l 288.361 365.852 m
288.361 365.852 l 288.361 365.852 m 220.379 330.107 l 220.379
330.107 m 220.379 330.107 l 220.379 330.107 m 220.379 330.107 l
220.379 330.107 m 262.871 307.765 l 262.871 307.765 m 262.871
307.765 l 262.871 307.765 m 262.871 307.765 l 262.871 307.765 m
199.696 274.548 l 199.696 274.548 m 199.696 274.548 l 199.696
274.548 m 199.696 274.548 l 199.696 274.548 m 149.629 300.873 l
149.629 300.873 m 149.629 300.873 l 149.629 300.873 m 149.629
300.873 l 149.629 300.873 m 202.461 328.652 l 202.461 328.652 m
202.461 328.652 l 202.461 328.652 m 202.461 328.652 l 202.461
328.652 m 262.871 296.889 l 262.871 296.889 m 262.871 296.889 l
262.871 296.889 m 262.871 296.889 l 262.871 296.889 m 220.379
274.546 l 220.379 274.546 m 220.379 274.546 l 220.379 274.546 m
220.379 274.546 l 220.379 274.546 m 291.125 237.348 l 291.125
237.348 m 291.125 237.348 l 291.125 237.348 m 291.125 237.348 l
291.125 237.348 m 333.621 259.692 l 333.621 259.692 m 333.621
259.692 l 333.621 259.692 m 333.621 259.692 l 333.621 259.692 m
273.218 291.452 l 273.218 291.452 m 273.218 291.452 l 273.218
291.452 m 273.218 291.452 l 273.218 291.452 m 220.379 263.670 l
220.379 263.670 m 220.379 263.670 l 220.379 263.670 m 220.379
263.670 l 220.379 263.670 m 270.439 237.348 l 270.439 237.348 m
270.439 237.348 l 270.439 237.348 m 270.439 237.348 l 270.439
237.348 m 333.621 270.569 l 333.621 270.569 m 333.621 270.569 l
333.621 270.569 m 333.621 270.569 l 333.621 270.569 m 291.129
292.911 l 291.129 292.911 m 291.129 292.911 l 291.129 292.911 m
291.129 292.911 l 291.129 292.911 m 359.104 328.652 l 359.104
328.652 m 359.104 328.652 l 359.104 328.652 m 359.104 328.652 l
359.104 328.652 m 404.371 304.851 l 404.371 304.851 m 404.371
304.851 l 404.371 304.851 m 404.371 304.851 l 404.371 304.851 m
346.739 274.548 l 346.739 274.548 m 346.739 274.548 l 346.739
274.548 m 346.739 274.548 l 346.739 274.548 m 291.129 303.788 l
291.129 303.788 m 291.129 303.788 l 291.129 303.788 m 291.129
303.788 l 291.129 303.788 m 338.418 328.652 l 338.418 328.652 m
338.418 328.652 l 338.418 328.652 m 338.418 328.652 l 338.418
328.652 m 404.371 293.974 l 404.371 293.974 m 404.371 293.974 l
404.371 293.974 m 404.371 293.974 l 404.371 293.974 m 361.879
271.632 l 361.879 271.632 m 361.879 271.632 l 361.879 271.632 m
361.879 271.632 l 361.879 271.632 m 427.082 237.348 l 427.082
237.348 m 427.082 237.348 l 427.082 237.348 m 427.082 237.348 l
427.082 237.348 m 475.121 262.607 l 475.121 262.607 m 475.121
262.607 l 475.121 262.607 m 475.121 262.607 l 475.121 262.607 m
420.260 291.452 l 420.260 291.452 m 420.260 291.452 l 420.260
291.452 m 420.260 291.452 l 420.260 291.452 m 361.879 260.755 l
361.879 260.755 m 361.879 260.755 l 361.879 260.755 m 361.879
260.755 l 361.879 260.755 m 406.397 237.348 l 406.397 237.348 m
406.397 237.348 l 406.397 237.348 m 406.397 237.348 l 406.397
237.348 m 475.121 273.483 l 475.121 273.483 m 475.121 273.483 l
475.121 273.483 m 475.121 273.483 l 475.121 273.483 m 432.629
295.825 l 432.629 295.825 m 432.629 295.825 l 432.629 295.825 m
432.629 295.825 l 432.629 295.825 m 495.061 328.652 l 495.061
328.652 m 495.061 328.652 l 495.061 328.652 m 495.061 328.652 l
495.061 328.652 m 545.871 301.936 l 545.871 301.936 m 545.871
301.936 l 545.871 301.936 m 545.871 301.936 l 545.871 301.936 m
493.782 274.548 l 493.782 274.548 m 493.782 274.548 l 493.782
274.548 m 493.782 274.548 l 493.782 274.548 m 432.629 306.702 l
432.629 306.702 m 432.629 306.702 l 432.629 306.702 m 432.629
306.702 l 432.629 306.702 m 475.121 329.044 l 475.121 329.044 m
475.121 329.044 l 475.121 329.044 m 475.121 329.044 l 475.121
329.044 m 405.117 365.852 l 405.117 365.852 m 405.117 365.852 l
405.117 365.852 m 405.117 365.852 l 405.117 365.852 m 361.879
343.117 l 361.879 343.117 m 361.879 343.117 l 361.879 343.117 m
361.879 343.117 l 361.879 343.117 m 421.540 311.748 l 421.540
311.748 m 421.540 311.748 l 421.540 311.748 m 421.540 311.748 l
421.540 311.748 m 475.121 339.921 l 475.121 339.921 m 475.121
339.921 l 475.121 339.921 m 475.121 339.921 l 475.121 339.921 m
425.803 365.852 l 425.803 365.852 m 425.803 365.852 l 425.803
365.852 m 425.803 365.852 l 425.803 365.852 m 361.879 332.241 l
361.879 332.241 m 361.879 332.241 l 361.879 332.241 m 361.879
332.241 l 361.879 332.241 m 404.371 309.898 l 404.371 309.898 m
404.371 309.898 l 404.371 309.898 m 404.371 309.898 l 404.371
309.898 m 337.139 274.548 l 337.139 274.548 m 337.139 274.548 l
337.139 274.548 m 337.139 274.548 l 337.139 274.548 m 291.129
298.740 l 291.129 298.740 m 291.129 298.740 l 291.129 298.740 m
291.129 298.740 l 291.129 298.740 m 348.018 328.652 l 348.018
328.652 m 348.018 328.652 l 348.018 328.652 m 348.018 328.652 l
348.018 328.652 m 404.371 299.022 l 404.371 299.022 m 404.371
299.022 l 404.371 299.022 m 404.371 299.022 l 404.371 299.022 m
357.825 274.548 l 357.825 274.548 m 357.825 274.548 l 357.825
274.548 m 357.825 274.548 l 357.825 274.548 m 291.129 309.616 l
291.129 309.616 m 291.129 309.616 l 291.129 309.616 m 291.129
309.616 l 291.129 309.616 m 333.621 331.959 l 333.621 331.959 m
333.621 331.959 l 333.621 331.959 m 333.621 331.959 l 333.621
331.959 m 269.160 365.852 l 269.160 365.852 m 269.160 365.852 l
269.160 365.852 m 269.160 365.852 l 269.160 365.852 m 220.379
340.203 l 220.379 340.203 m 220.379 340.203 l 220.379 340.203 m
220.379 340.203 l 220.379 340.203 m 274.497 311.748 l 274.497
311.748 m 274.497 311.748 l 274.497 311.748 m 274.497 311.748 l
274.497 311.748 m 333.621 342.835 l 333.621 342.835 m 333.621
342.835 l 333.621 342.835 m 333.621 342.835 l 333.621 342.835 m
289.846 365.852 l 289.846 365.852 m 289.846 365.852 l 289.846
365.852 m 289.846 365.852 l 289.846 365.852 m 220.379 329.327 l
220.379 329.327 m 220.379 329.327 l 220.379 329.327 m 220.379
329.327 l 220.379 329.327 m 262.871 306.984 l 262.871 306.984 m
262.871 306.984 l 262.871 306.984 m 262.871 306.984 l 262.871
306.984 m 201.182 274.548 l 201.182 274.548 m 201.182 274.548 l
201.182 274.548 m 201.182 274.548 l 201.182 274.548 m 149.629
301.654 l 149.629 301.654 m 149.629 301.654 l 149.629 301.654 m
149.629 301.654 l 149.629 301.654 m 200.976 328.652 l 200.976
328.652 m 200.976 328.652 l 200.976 328.652 m 200.976 328.652 l
200.976 328.652 m 262.871 296.108 l 262.871 296.108 m 262.871
296.108 l 262.871 296.108 m 262.871 296.108 l 262.871 296.108 m
220.379 273.765 l 220.379 273.765 m 220.379 273.765 l 220.379
273.765 m 220.379 273.765 l 220.379 273.765 m 289.640 237.348 l
289.640 237.348 m 289.640 237.348 l 289.640 237.348 m 289.640
237.348 l 289.640 237.348 m 333.621 260.473 l 333.621 260.473 m
333.621 260.473 l 333.621 260.473 m 333.621 260.473 l 333.621
260.473 m 274.703 291.452 l 274.703 291.452 m 274.703 291.452 l
274.703 291.452 m 274.703 291.452 l 274.703 291.452 m 220.379
262.889 l 220.379 262.889 m 220.379 262.889 l 220.379 262.889 m
220.379 262.889 l 220.379 262.889 m 268.954 237.348 l 268.954
237.348 m 268.954 237.348 l 268.954 237.348 m 268.954 237.348 l
268.954 237.348 m 333.621 271.350 l 333.621 271.350 m 333.621
271.350 l 333.621 271.350 m 333.621 271.350 l 333.621 271.350 m
291.129 293.692 l 291.129 293.692 m 291.129 293.692 l 291.129
293.692 m 291.129 293.692 l 291.129 293.692 m 357.619 328.652 l
357.619 328.652 m 357.619 328.652 l 357.619 328.652 m 357.619
328.652 l 357.619 328.652 m 404.371 304.070 l 404.371 304.070 m
404.371 304.070 l 404.371 304.070 m 404.371 304.070 l stroke 404.371
304.070 m 348.224 274.548 l 348.224 274.548 m 348.224 274.548 l
348.224 274.548 m 348.224 274.548 l 348.224 274.548 m 291.129
304.568 l 291.129 304.568 m 291.129 304.568 l 291.129 304.568 m
291.129 304.568 l 291.129 304.568 m 336.933 328.652 l 336.933
328.652 m 336.933 328.652 l 336.933 328.652 m 336.933 328.652 l
336.933 328.652 m 404.371 293.193 l 404.371 293.193 m 404.371
293.193 l 404.371 293.193 m 404.371 293.193 l 404.371 293.193 m
361.879 270.851 l 361.879 270.851 m 361.879 270.851 l 361.879
270.851 m 361.879 270.851 l 361.879 270.851 m 425.597 237.348 l
425.597 237.348 m 425.597 237.348 l 425.597 237.348 m 425.597
237.348 l 425.597 237.348 m 475.121 263.387 l 475.121 263.387 m
475.121 263.387 l 475.121 263.387 m 475.121 263.387 l 475.121
263.387 m 421.746 291.452 l 421.746 291.452 m 421.746 291.452 l
421.746 291.452 m 421.746 291.452 l 421.746 291.452 m 361.879
259.974 l 361.879 259.974 m 361.879 259.974 l 361.879 259.974 m
361.879 259.974 l 361.879 259.974 m 404.911 237.348 l 404.911
237.348 m 404.911 237.348 l 404.911 237.348 m 404.911 237.348 l
404.911 237.348 m 475.121 274.264 l 475.121 274.264 m 475.121
274.264 l 475.121 274.264 m 475.121 274.264 l 475.121 274.264 m
432.629 296.606 l 432.629 296.606 m 432.629 296.606 l 432.629
296.606 m 432.629 296.606 l 432.629 296.606 m 493.576 328.652 l
493.576 328.652 m 493.576 328.652 l 493.576 328.652 m 493.576
328.652 l 493.576 328.652 m 545.871 301.155 l 545.871 301.155 m
545.871 301.155 l 545.871 301.155 m 545.871 301.155 l 545.871
301.155 m 495.267 274.548 l 495.267 274.548 m 495.267 274.548 l
495.267 274.548 m 495.267 274.548 l 495.267 274.548 m 432.629
307.483 l 432.629 307.483 m 432.629 307.483 l 432.629 307.483 m
432.629 307.483 l 432.629 307.483 m 475.121 329.825 l 475.121
329.825 m 475.121 329.825 l 475.121 329.825 m 475.121 329.825 l
475.121 329.825 m 406.603 365.852 l 406.603 365.852 m 406.603
365.852 l 406.603 365.852 m 406.603 365.852 l 406.603 365.852 m
361.879 342.336 l 361.879 342.336 m 361.879 342.336 l 361.879
342.336 m 361.879 342.336 l 361.879 342.336 m 420.054 311.748 l
420.054 311.748 m 420.054 311.748 l 420.054 311.748 m 420.054
311.748 l 420.054 311.748 m 475.121 340.702 l 475.121 340.702 m
475.121 340.702 l 475.121 340.702 m 475.121 340.702 l 475.121
340.702 m 427.288 365.852 l 427.288 365.852 m 427.288 365.852 l
427.288 365.852 m 427.288 365.852 l 427.288 365.852 m 361.879
331.460 l 361.879 331.460 m 361.879 331.460 l 361.879 331.460 m
361.879 331.460 l 361.879 331.460 m 404.371 309.118 l 404.371
309.118 m 404.371 309.118 l 404.371 309.118 m 404.371 309.118 l
404.371 309.118 m 338.624 274.548 l 338.624 274.548 m 338.624
274.548 l 338.624 274.548 m 338.624 274.548 l 338.624 274.548 m
291.129 299.521 l 291.129 299.521 m 291.129 299.521 l 291.129
299.521 m 291.129 299.521 l 291.129 299.521 m 346.533 328.652 l
346.533 328.652 m 346.533 328.652 l 346.533 328.652 m 346.533
328.652 l 346.533 328.652 m 404.371 298.241 l 404.371 298.241 m
404.371 298.241 l 404.371 298.241 m 404.371 298.241 l 404.371
298.241 m 359.310 274.548 l 359.310 274.548 m 359.310 274.548 l
359.310 274.548 m 359.310 274.548 l 359.310 274.548 m 291.129
310.397 l 291.129 310.397 m 291.129 310.397 l 291.129 310.397 m
291.129 310.397 l 291.129 310.397 m 333.621 332.740 l 333.621
332.740 m 333.621 332.740 l 333.621 332.740 m 333.621 332.740 l
333.621 332.740 m 270.645 365.852 l 270.645 365.852 m 270.645
365.852 l 270.645 365.852 m 270.645 365.852 l 270.645 365.852 m
220.379 339.422 l 220.379 339.422 m 220.379 339.422 l 220.379
339.422 m 220.379 339.422 l 220.379 339.422 m 273.012 311.748 l
273.012 311.748 m 273.012 311.748 l 273.012 311.748 m 273.012
311.748 l 273.012 311.748 m 333.621 343.616 l 333.621 343.616 m
333.621 343.616 l 333.621 343.616 m 333.621 343.616 l 333.621
343.616 m 291.129 365.959 l 291.129 365.959 m 291.129 365.959 l
291.129 365.959 m 291.129 365.959 l 291.129 365.959 m 361.676
403.052 l 361.676 403.052 m 361.676 403.052 l 361.676 403.052 m
361.676 403.052 l 361.676 403.052 m 404.371 380.603 l 404.371
380.603 m 404.371 380.603 l 404.371 380.603 m 404.371 380.603 l
404.371 380.603 m 344.167 348.948 l 344.167 348.948 m 344.167
348.948 l 344.167 348.948 m 344.167 348.948 l 344.167 348.948 m
291.129 376.835 l 291.129 376.835 m 291.129 376.835 l 291.129
376.835 m 291.129 376.835 l 291.129 376.835 m 340.990 403.052 l
340.990 403.052 m 340.990 403.052 l 340.990 403.052 m 340.990
403.052 l 340.990 403.052 m 404.371 369.727 l 404.371 369.727 m
404.371 369.727 l 404.371 369.727 m 404.371 369.727 l 404.371
369.727 m 361.879 347.384 l 361.879 347.384 m 361.879 347.384 l
361.879 347.384 m 361.879 347.384 l 361.879 347.384 m 429.655
311.748 l 429.655 311.748 m 429.655 311.748 l 429.655 311.748 m
429.655 311.748 l 429.655 311.748 m 475.121 335.654 l 475.121
335.654 m 475.121 335.654 l 475.121 335.654 m 475.121 335.654 l
475.121 335.654 m 417.688 365.852 l 417.688 365.852 m 417.688
365.852 l 417.688 365.852 m 417.688 365.852 l 417.688 365.852 m
361.879 336.508 l 361.879 336.508 m 361.879 336.508 l 361.879
336.508 m 361.879 336.508 l 361.879 336.508 m 408.969 311.748 l
408.969 311.748 m 408.969 311.748 l 408.969 311.748 m 408.969
311.748 l 408.969 311.748 m 475.121 346.530 l 475.121 346.530 m
475.121 346.530 l 475.121 346.530 m 475.121 346.530 l 475.121
346.530 m 432.629 368.873 l 432.629 368.873 m 432.629 368.873 l
432.629 368.873 m 432.629 368.873 l 432.629 368.873 m 497.633
403.052 l 497.633 403.052 m 497.633 403.052 l 497.633 403.052 m
497.633 403.052 l 497.633 403.052 m 545.871 377.689 l 545.871
377.689 m 545.871 377.689 l 545.871 377.689 m 545.871 377.689 l
545.871 377.689 m 491.209 348.948 l 491.209 348.948 m 491.209
348.948 l 491.209 348.948 m 491.209 348.948 l 491.209 348.948 m
432.629 379.749 l 432.629 379.749 m 432.629 379.749 l 432.629
379.749 m 432.629 379.749 l 432.629 379.749 m 476.948 403.052 l
476.948 403.052 m 476.948 403.052 l 476.948 403.052 m 476.948
403.052 l 476.948 403.052 m 545.871 366.812 l 545.871 366.812 m
545.871 366.812 l 545.871 366.812 m 545.871 366.812 l 545.871
366.812 m 503.379 344.470 l 503.379 344.470 m 503.379 344.470 l
503.379 344.470 m 503.379 344.470 l 503.379 344.470 m 565.612
311.748 l 565.612 311.748 m 565.612 311.748 l 565.612 311.748 m
565.612 311.748 l 565.612 311.748 m 616.621 338.568 l 616.621
338.568 m 616.621 338.568 l 616.621 338.568 m 616.621 338.568 l
616.621 338.568 m 564.731 365.852 l 564.731 365.852 m 564.731
365.852 l 564.731 365.852 m 564.731 365.852 l 564.731 365.852 m
503.379 333.593 l 503.379 333.593 m 503.379 333.593 l 503.379
333.593 m 503.379 333.593 l 503.379 333.593 m 545.871 311.251 l
545.871 311.251 m 545.871 311.251 l 545.871 311.251 m 545.871
311.251 l 545.871 311.251 m 476.066 274.548 l 476.066 274.548 m
476.066 274.548 l 476.066 274.548 m 476.066 274.548 l 476.066
274.548 m 432.629 297.387 l 432.629 297.387 m 432.629 297.387 l
432.629 297.387 m 432.629 297.387 l 432.629 297.387 m 492.091
328.652 l 492.091 328.652 m 492.091 328.652 l 492.091 328.652 m
492.091 328.652 l 492.091 328.652 m 545.871 300.375 l 545.871
300.375 m 545.871 300.375 l 545.871 300.375 m 545.871 300.375 l
545.871 300.375 m 496.752 274.548 l 496.752 274.548 m 496.752
274.548 l 496.752 274.548 m 496.752 274.548 l 496.752 274.548 m
432.629 308.264 l 432.629 308.264 m 432.629 308.264 l 432.629
308.264 m 432.629 308.264 l 432.629 308.264 m 475.121 330.606 l
475.121 330.606 m 475.121 330.606 l 475.121 330.606 m 475.121
330.606 l 475.121 330.606 m 408.088 365.852 l 408.088 365.852 m
408.088 365.852 l 408.088 365.852 m 408.088 365.852 l 408.088
365.852 m 361.879 341.556 l 361.879 341.556 m 361.879 341.556 l
361.879 341.556 m 361.879 341.556 l 361.879 341.556 m 418.569
311.748 l 418.569 311.748 m 418.569 311.748 l 418.569 311.748 m
418.569 311.748 l 418.569 311.748 m 475.121 341.483 l 475.121
341.483 m 475.121 341.483 l 475.121 341.483 m 475.121 341.483 l
475.121 341.483 m 428.774 365.852 l 428.774 365.852 m 428.774
365.852 l 428.774 365.852 m 428.774 365.852 l 428.774 365.852 m
361.879 330.679 l 361.879 330.679 m 361.879 330.679 l 361.879
330.679 m 361.879 330.679 l 361.879 330.679 m 404.371 308.337 l
404.371 308.337 m 404.371 308.337 l 404.371 308.337 m 404.371
308.337 l 404.371 308.337 m 340.109 274.548 l 340.109 274.548 m
340.109 274.548 l 340.109 274.548 m 340.109 274.548 l 340.109
274.548 m 291.129 300.302 l 291.129 300.302 m 291.129 300.302 l
291.129 300.302 m 291.129 300.302 l 291.129 300.302 m 345.048
328.652 l 345.048 328.652 m 345.048 328.652 l 345.048 328.652 m
345.048 328.652 l 345.048 328.652 m 404.371 297.460 l 404.371
297.460 m 404.371 297.460 l 404.371 297.460 m 404.371 297.460 l
404.371 297.460 m 360.795 274.548 l 360.795 274.548 m 360.795
274.548 l 360.795 274.548 m 360.795 274.548 l 360.795 274.548 m
291.129 311.178 l 291.129 311.178 m 291.129 311.178 l 291.129
311.178 m 291.129 311.178 l 291.129 311.178 m 333.621 333.521 l
333.621 333.521 m 333.621 333.521 l 333.621 333.521 m 333.621
333.521 l 333.621 333.521 m 272.131 365.852 l 272.131 365.852 m
272.131 365.852 l stroke 272.131 365.852 m 272.131 365.852 l 272.131
365.852 m 220.379 338.641 l 220.379 338.641 m 220.379 338.641 l
220.379 338.641 m 220.379 338.641 l 220.379 338.641 m 271.527
311.748 l 271.527 311.748 m 271.527 311.748 l 271.527 311.748 m
271.527 311.748 l 271.527 311.748 m 333.621 344.397 l 333.621
344.397 m 333.621 344.397 l 333.621 344.397 m 333.621 344.397 l
333.621 344.397 m 291.129 366.739 l 291.129 366.739 m 291.129
366.739 l 291.129 366.739 m 291.129 366.739 l 291.129 366.739 m
360.191 403.052 l 360.191 403.052 m 360.191 403.052 l 360.191
403.052 m 360.191 403.052 l 360.191 403.052 m 404.371 379.822 l
404.371 379.822 m 404.371 379.822 l 404.371 379.822 m 404.371
379.822 l 404.371 379.822 m 345.652 348.948 l 345.652 348.948 m
345.652 348.948 l 345.652 348.948 m 345.652 348.948 l 345.652
348.948 m 291.129 377.616 l 291.129 377.616 m 291.129 377.616 l
291.129 377.616 m 291.129 377.616 l 291.129 377.616 m 339.505
403.052 l 339.505 403.052 m 339.505 403.052 l 339.505 403.052 m
339.505 403.052 l 339.505 403.052 m 404.371 368.946 l 404.371
368.946 m 404.371 368.946 l 404.371 368.946 m 404.371 368.946 l
404.371 368.946 m 361.879 346.603 l 361.879 346.603 m 361.879
346.603 l 361.879 346.603 m 361.879 346.603 l 361.879 346.603 m
428.170 311.748 l 428.170 311.748 m 428.170 311.748 l 428.170
311.748 m 428.170 311.748 l 428.170 311.748 m 475.121 336.435 l
475.121 336.435 m 475.121 336.435 l 475.121 336.435 m 475.121
336.435 l 475.121 336.435 m 419.173 365.852 l 419.173 365.852 m
419.173 365.852 l 419.173 365.852 m 419.173 365.852 l 419.173
365.852 m 361.879 335.727 l 361.879 335.727 m 361.879 335.727 l
361.879 335.727 m 361.879 335.727 l 361.879 335.727 m 407.484
311.748 l 407.484 311.748 m 407.484 311.748 l 407.484 311.748 m
407.484 311.748 l 407.484 311.748 m 475.121 347.311 l 475.121
347.311 m 475.121 347.311 l 475.121 347.311 m 475.121 347.311 l
475.121 347.311 m 432.629 369.654 l 432.629 369.654 m 432.629
369.654 l 432.629 369.654 m 432.629 369.654 l 432.629 369.654 m
496.148 403.052 l 496.148 403.052 m 496.148 403.052 l 496.148
403.052 m 496.148 403.052 l 496.148 403.052 m 545.871 376.908 l
545.871 376.908 m 545.871 376.908 l 545.871 376.908 m 545.871
376.908 l 545.871 376.908 m 492.695 348.948 l 492.695 348.948 m
492.695 348.948 l 492.695 348.948 m 492.695 348.948 l 492.695
348.948 m 432.629 380.530 l 432.629 380.530 m 432.629 380.530 l
432.629 380.530 m 432.629 380.530 l 432.629 380.530 m 475.463
403.052 l 475.463 403.052 m 475.463 403.052 l 475.463 403.052 m
475.463 403.052 l 475.463 403.052 m 545.871 366.031 l 545.871
366.031 m 545.871 366.031 l 545.871 366.031 m 545.871 366.031 l
545.871 366.031 m 503.379 343.689 l 503.379 343.689 m 503.379
343.689 l 503.379 343.689 m 503.379 343.689 l 503.379 343.689 m
564.127 311.748 l 564.127 311.748 m 564.127 311.748 l 564.127
311.748 m 564.127 311.748 l 564.127 311.748 m 616.621 339.349 l
616.621 339.349 m 616.621 339.349 l 616.621 339.349 m 616.621
339.349 l 616.621 339.349 m 566.216 365.852 l stroke copypage

